COMFYCLAW: Self-Evolving Skill Harnesses for Image Generation Workflows

Agents are increasingly used to construct workflows and assist humans in completing recurring tasks more efficiently. As these workflows become repeated and domain-specific, agent memory and reusable skills become increasingly important: agents should be able to recall workflow patterns, execution constraints, and user preferences from previous runs. We study this problem in workflow-based image generation and introduce COMFYCLAW, an agentic skill evolution harness for controlling ComfyUI workflows. COMFYCLAW formulates workflow construction as typed graph editing, exposes tools organized by construction stage, automatically reverts invalid edits, and uses a region-level vision-language model (VLM) verifier to translate visual failures into actionable repair suggestions. The framework further evolves a progressively disclosed skill library, where trajectories, execution errors, and verifier feedback from previous runs are distilled into reusable Agent Skills. Across four benchmark splits, three agent models, and two image backbones, COMFYCLAW achieves the best average image-generation evaluation score across all six agent configurations, outperforming a verifier-only baseline without skill evolution. Human annotations further show that annotators prefer COMFYCLAW over variants without skill evolution. Our results suggest that skill evolution is an effective mechanism for improving agent reliability and performance in recurring visual workflow construction.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The abstract and Section~\ref{sec:introduction} clearly identify the four \ours{} harness mechanisms and state the central empirical claim that self-evolving workflow skills paired with verifier-grounded repair outperform both one-shot workflow generation and verifier-only refinement. These claims are quantitatively supported by the four-benchmark evaluation (Table~\ref{tab:results1}) and human annotation study (Table~\ref{tab:qualitative_evals}) in Section~\ref{sec:results}, with additional characterization of evolved-skill read statistics (Table~\ref{tab:evolved}) and workflow-event breakdown (Table~\ref{tab:modification-breakdown}) provided in Appendix~\ref{app:skill-read-stats}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}.
    \item[] Justification: It is discussed in Section~\ref{sec:limitation}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}.
    \item[] Justification: There is no theory assumption and proof involved.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}.
    \item[] Justification: Section~\ref{sec:method} provides the harness algorithm. Section~\ref{sec:results} provides all benchmarks with prompt counts, agent models, image backbones, evaluation metrics, the judge model (Qwen3-VL-8B-Instruct), both baselines, and the GPU hardware (RTX PRO 6000 Blackwell, 96~GB). Appendix~\ref{app:prompts:verifier} provides the prompt template for agents to reproduce the agent workflow control pipeline.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
         \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}.
    \item[] Justification: All four benchmarks (GenEval~2, DPG-Bench, OneIG-EN, OneIG-ZH) are publicly available, and the agent models, image backbones, and judge model are named and cited. Selected demo results are included in the supplemental materials. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{}.
    \item[] Justification: Section~\ref{sec:results} specifies the four benchmark splits with prompt counts (${\approx}4{,}300$ prompts total), three agent models, two image backbones, 17 base tools, four predefined skills, per-benchmark evaluation metrics, the judge model (Qwen3-VL-8B-Instruct), both baseline conditions, and GPU hardware. Appendix~\ref{app:user_study} discusses the user study numbers and costs.
    % Appendix~\ref{app:user_study} discusses the user study numbers and costs.
    % Section~\ref{sec:method} specifies the reward weights ($w_{\mathrm{req}}{=}0.6$, $w_{\mathrm{det}}{=}0.4$), complexity penalty ($\lambda{=}0.02$), and discount factor ($\gamma{=}0$). The loop hyperparameters ($T$, $\tau$, $r_{\max}$, $\kappa_{\max}$) and LLM generation settings are not yet reported. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{}.
    \item[] Justification: Benchmark scores in Table~\ref{tab:results1} and human ratings in Table~\ref{tab:qualitative_evals} are reported as point estimates. Obtaining multiple independent seeds for the full agentic harness across ${\approx}4{,}300$ prompts and six agent--backbone configurations would require prohibitive additional compute. No statistical results are needed to report for the results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}.
    \item[] Justification: Section~\ref{sec:results} reports that all experiments were conducted on an RTX PRO 6000 Blackwell GPU with 96~GB memory. 
    % Per-configuration wall-clock time, total GPU-hours, and compute attributable to preliminary or discarded runs are not reported. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The work uses publicly available benchmarks and models, does not collect personal data, and the human annotation study involves aggregate image-quality ratings with minimal participant risk. Annotators are compensated above minimum wage (see Item~15). Author anonymity is maintained in the submission.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The introduction and related work motivate accessibility benefits for non-expert users of ComfyUI. Section~\ref{sec:limitation} discusses the broader impact of using agents to automate ComfyUI workflows for content creation, covering both opportunities for non-expert users and risks of misuse.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}.
    \item[] Justification: The paper presents a harness framework that wraps existing, publicly released image-generation models (z-image-turbo, LongCat-Image) and does not introduce a new pretrained generative model or scraped dataset. No new high-risk generative asset is released with this submission.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}.
    \item[] Justification: All datasets, models, and tools are credited via citations. The two LoRA weights used with z-image-turbo are identified by URL in Section~\ref{sec:results}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}.
    \item[] Justification: The paper does not release new assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)?
    \item[] Answer: \answerYes{}.
    \item[] Justification: Section~\ref{sec:results} describes a human qualitative evaluation in which two annotators rated 2{,}400 AI-generated images on a 1--5 Likert scale at \$0.10 per image. The full annotation guidelines, rating interface, and recruitment procedure are included in Appendix~\ref{app:user_study}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The Institutional Review Board (IRB) has reviewed and exempted the annotation protocol (Appendix~\ref{app:user_study}). Annotators are compensated at \$0.10 per image rated, above local minimum wage. Participant risk is minimal, as the task involves rating AI-generated images with no collection of personal information.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerYes{}.
    \item[] Justification: LLM and VLM models are core, non-standard components of \ours{}: they serve as the workflow-control agent, region-level verifier, and skill-evolution agent. Sections~\ref{sec:method} and~\ref{sec:results} describe each role in detail and enumerate all model versions (Claude~Sonnet~4.5, Qwen-3.6-35B-A3B, and Gemma-4-E4B-it as agents; Qwen3-VL-8B-Instruct as the benchmark judge).
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}


==> sections/full.tex <==

% \section{Introduction}
% \label{sec:introduction}

% % \wxy{the intro need to be fully rewrite, a few things, 1. we don't need to list many related products, or acutal tools, used, need to focus on high-level infra; 2. it might be better to motivated by why agentic workflow is promising, and what's teh current drawback of workflow in image creation}


% % Language-model agents are increasingly expected to operate software rather than
% % merely answer questions. Across software engineering, desktop control, embodied
% % AI, games, web automation, and data analysis, the common abstraction is
% % \emph{agentic workflow control}: an agent must select tools, update external
% % state, interpret execution failures, judge partial outputs, and reuse experience
% % from prior attempts~\cite{wang2023voyager,wu2024copilot,xie2024osworld,workarena2024,chezelles2025browsergym,xu2025agents,wu2026saber}.
% % This abstraction is promising because it turns expert procedures into
% % inspectable, repeatable interaction traces. It is also difficult because the
% % agent must manage a long-horizon control loop whose errors are not limited to
% % bad language outputs; a single wrong operation can invalidate the external
% % workflow.

% % Language-model agents are increasingly used to control external workflows rather than only produce textual answers~\cite{wang2023voyager,wu2024copilot,xie2024osworld,workarena2024,chezelles2025browsergym,xu2025agents,wu2026saber}. 
% % This shift is promising because workflows turn expert procedures into executable, inspectable, and reusable artifacts~\cite{gal2024comfygen}. 
% % However, workflow control is much harder than answer generation: the agent must choose valid actions, update external state, interpret runtime feedback, and recover from failures over a long horizon. 
% % A single invalid operation can break the workflow, and the error is often only visible after execution~\cite{su2026comfysearch}.


% % Language-model agents are moving from answering questions to controlling executable workflows. In \emph{agentic workflow control}, an agent must select tools, update external state, interpret execution failures, judge partial outputs, and reuse experience from prior attempts~\cite{wang2023voyager,wu2024copilot,xie2024osworld,workarena2024,chezelles2025browsergym,xu2025agents,wu2026saber}.  
% % %
% % This shift is promising because workflows expose expert procedures as inspectable, repeatable traces rather than one-off outputs~\cite{gal2024comfygen}. 
% % %
% % However, workflow control is much harder than answer generation: the agent must choose valid actions, update external state, interpret runtime feedback, and recover from failures over a long horizon. 
% % %
% % A single invalid operation can break the workflow, and the error is often only visible after execution~\cite{su2026comfysearch}.

% \emph{Agentic workflow control} is useful across many everyday tasks, and visual
% generation is a representative case where agents must control complex image and video pipelines~\cite{xu2025comfyui}.
% %
% Prompt-only interfaces are easy to use, but provide limited control over
% intermediate components, hyperparameters, and failure repair~\cite{cao2025controllable}.
% %
% Workflow-based systems such as ComfyUI expose generation as an editable
% pipeline, enabling users to inspect and modify text encoders, conditioning,
% sampling, refinement, regional editing, and inpainting
% steps~\cite{gal2024comfygen,huang2025comfygpt}.
% %
% ComfyUI's large open-source ecosystem, including over 100K GitHub stars and
% 800+ custom-node authors, shows strong demand for controllable creative
% workflows~\cite{comfyui_registry}.
% %
% However, this flexibility also makes workflow construction difficult for beginners, motivating agents that can automatically build, refine, and repair workflows to help users learn these tools and automate complex generation tasks~\cite{gal2024comfygen,sobania2024comfygi}.






% In \emph{agentic workflow control}, agents operate on expert procedures as
% inspectable, repeatable traces rather than producing one-off
% outputs~\cite{wang2023voyager,wu2024copilot,xie2024osworld,workarena2024,chezelles2025browsergym,xu2025agents,gal2024comfygen}.
% %
% This is challenging because agents must interact with an execution environment through a harness, where one invalid action can break the workflow and errors may appear only after execution~\cite{pan2026natural,su2026comfysearch}.
% %
% Existing workflow-generation agents reduce this burden by generating or
% refining graphs from natural language~\cite{xu2025comfyui,jiang2026genagent,xue2025comfybench}, while systems such as GEMS show that closed-loop refinement,
% memory, and skills can improve multimodal generation~\cite{he2026gems}.
% %
% However, these systems often treat the interface and skill library as static or passively accumulated components.
% %
% Thus, repeated failures may be repaired locally during a run, but without a
% mechanism for validating and storing these fixes as reusable skills, they cannot be systematically reused in later tasks~\cite{wang2023voyager}.






% %
% % This interface makes generation more controllable, but shifts the burden from prompt writing to procedure construction: the agent must choose compatible components, respect model constraints, localize visual failures, and repair the graph without breaking execution. 


% % Image-creation workflows expose this tension in a particularly concrete form.
% % Node-graph systems such as ComfyUI~\cite{comfyanonymous2023comfyui} make
% % generation pipelines modular and inspectable, but valid graph construction
% % requires tacit knowledge about node compatibility, model-specific constraints,
% % and community conventions. For beginners, the barrier is therefore not simply
% % ``how to write a better prompt,'' but how to assemble, diagnose, and adapt a
% % working procedure. Existing ComfyUI agents reduce this barrier by generating or
% % refining workflows from natural language
% % ~\cite{gal2024comfygen,huang2025comfygpt,xu2025comfyui,jiang2026genagent,xue2025comfybench};
% % GEMS further shows that memory, skills, and verifier-guided refinement can make
% % multimodal generation more agent-native~\cite{he2026gems}. These advances point
% % to a broader question that is not specific to image quality: what infrastructure
% % makes an agent reliable at controlling the workflow itself?


% % Image-creation workflows expose this tension in a particularly concrete form.
% % Prompt-only generation is easy to use but offers limited control, while workflow-based generation allows users to compose conditioning, sampling, refinement, regional editing, LoRA modules, and inpainting into an explicit graph. 
% % This graph interface makes generation more controllable and inspectable, but it also requires procedural knowledge about component compatibility, model constraints, visual failure localization, and graph repair. 
% % Existing workflow-generation agents reduce this burden by producing or refining executable graphs from natural language, but they mostly optimize the current run. 
% % The tool interface and skill library are usually fixed, so repeated failures do not reliably become validated procedures that can be reused in later tasks.

% % Image creation provides a concrete instance of this control problem. 
% % Prompt-only generation is easy to use, but offers little structure for controlling intermediate decisions or repairing failures~\cite{cao2025controllable}. 
% % %
% % % Workflow-based generation exposes this structure as an executable graph, where users compose conditioning, sampling, refinement, regional editing, LoRA modules, and inpainting. 
% % %
% % Workflow-based generation instead exposes the generation process as an editable pipeline, where intermediate choices such as conditioning, sampling, refinement, regional editing, and inpainting can be inspected and modified~\cite{gal2024comfygen,huang2025comfygpt}.
% % %
% % This graph interface makes generation more controllable and inspectable, but shifts the burden from prompt writing to procedure construction: the agent must reason about component compatibility, model constraints, localized visual failures, and graph repair. 
% % Existing workflow-generation agents~\cite{xu2025comfyui,jiang2026genagent,xue2025comfybench} reduce this burden by producing or refining graphs from natural language, but they mostly optimize the current run. 
% % Their tool interfaces and skill libraries are usually fixed, so repeated failures do not reliably become validated procedures that can be reused in later tasks.


% % Existing workflow-generation agents reduce this burden by producing or refining graphs from natural language, but they mostly optimize the current run. 
% % Recent systems such as GEMS further show that closed-loop refinement, memory, and skills can improve multimodal generation~\citep{gems}. 
% % However, the control interface and skill library are still largely treated as fixed or accumulated components, rather than as testable parts of the workflow-control system. 
% % As a result, repeated failures do not reliably become validated procedures that can be reused in later tasks.




% % \wxy{the flow here is confusing, why we see this is two together? it look like there's no strong enough interconnection between teh two}
% % Reliable workflow control requires two coupled capabilities. The first is a
% % \emph{harness}: the external structure that exposes tools, memory, feedback, and
% % state transitions to an otherwise general model
% % \cite{madaan2023self,shinn2023reflexion,young2025effective,lou2026autoharness,lee2026meta,xu2026agent}.
% % The second is \emph{skill management}: the mechanism that turns repeated
% % trajectories into reusable procedural knowledge
% % \cite{wang2023voyager,wu2025evolver,xia2026skillrl,ni2026trace2skill,zhai2025agentevolver,gao2025survey,fang2025comprehensive}.
% % These capabilities are interdependent. A harness without evolving skills can
% % repair the current run but repeatedly makes the same future mistakes; evolving
% % skills without a disciplined harness can store brittle instructions that are
% % mis-triggered, invalid, or needlessly complex. Existing workflow-generation
% % agents largely keep this coupling fixed: they improve a candidate workflow
% % during inference, but the tool interface and skill library are usually authored
% % beforehand and not validated as learnable components. We therefore study the
% % following question: \emph{how can verifier feedback support both immediate
% % workflow repair and long-term self-evolution of the agent's skill library?}

% Recent work has shown growing interest in agent harnesses~\cite{lou2026autoharness}, memory systems~\cite{xu2025mem, zhang2026memrl},
% skill management~\cite{xia2026skillrl,yu2025polyskill}, and self-evolving agents~\cite{wu2026coevolvingllmdecisionskill} for workflow control.
% %
% These systems enable agents to execute commands, use tools, control workflows,
% and complete complex tasks by accumulating reusable experience.
% %
% General-purpose agent frameworks such as OpenClaw~\cite{openclaw2026} and
% Hermes-Agent~\cite{nousresearch2026hermesagent}, as well as automated research
% systems such as AutoResearch~\cite{karpathy2026autoresearch}, illustrate how
% memory and skills can support long-horizon workflow execution.
% %
% A parallel line of work studies self-evolving agents that improve through
% trial and error by interacting with an environment, receiving feedback, and
% updating their behavior from accumulated experience~\cite{wu2025evolver,xiang2026systematic,huang2025r,zhang2026memskill,he2026active}.
% %
% For image-generation workflow control, however, neither an agent harness nor
% static skill management is sufficient on its own.
% %
% A harness makes each workflow edit executable, observable, and recoverable,
% while skill management preserves useful procedures across tasks.
% %
% Without a disciplined harness, skills can become brittle text instructions that
% are mis-triggered, invalid for the current graph, or unnecessarily complex.
% %
% Without evolving skills, successful repairs remain local to a single run and do
% not improve future workflow construction.
% %
% Thus, the central challenge is not only to refine a workflow during one run,
% but also to use verifier feedback from that run to improve future control.
% %


% This motivates our question: \emph{can verifier feedback support both immediate
% workflow repair and the long-term evolution of a reusable skill library?}
% %
% Inspired by agentic workflow control and self-evolution, we propose \ours{}, a
% self-evolving framework for controlling image-generation workflows.
% %
% \ours{} integrates three components.
% %
% First, a harness represents workflow construction as typed graph edits, exposes
% tools through a stage-gated router, and uses rollback to recover from invalid
% edits~\cite{madaan2023self,shinn2023reflexion,young2025effective,lou2026autoharness,lee2026meta,xu2026agent}.
% %
% Second, a region-level VLM verifier converts visual failures into localized
% repair suggestions, allowing the agent to refine workflows using both verifier
% and runtime feedback.
% %
% Third, a progressively disclosed skill library converts successful
% trajectories, execution errors, and verifier feedback into reusable
% Agent~Skills, which are committed only after validation under a
% graph-complexity prior~\cite{wang2023voyager,wu2025evolver,xia2026skillrl,ni2026trace2skill,zhai2025agentevolver,gao2025survey,fang2025comprehensive}.

% We evaluate \ours{} with three agents, Claude-Sonnet-4.5~\cite{anthropic2025claude}, Gemma-4-E4B-it~\cite{gemma4_2026}, and Qwen-3.6-35B-A3B~\cite{qwen3}, on two image-generation models, LongCat-Image~\cite{team2025longcat} and Z-Image-Turbo~\cite{zimage2025}. 
% % 
% Across these settings, \ours{} outperforms agent harness workflow control without skill evolution by an average of 4 points out of 100, and outperforms agent workflow control without refinement by 10 points. 
% % 
% We further conduct user annotation on 2{,}400 randomly selected images, where users prefer \ours{} over both ablations on average.

% To study workflow repair and skill evolution together, we need a setting where an agent's decisions can be evaluated beyond the final output. ComfyUI workflow synthesis provides such a setting: each workflow is an executable graph, so invalid edits are rejected by the runtime, rendered images can be checked against decomposed visual requirements, and candidate skills can be tested on held-out prompts before entering the library.
% %
% In this paper, we introduce \ours{}, an agentic harness around an \emph{unmodified} ComfyUI runtime. \ours{} represents workflow construction as typed graph edits, exposes tools through a stage-gated router, uses rollback to recover from invalid edits, and applies a region-level VLM verifier to convert visual failures into localized repair suggestions. It also maintains a progressively disclosed skill library, where successful trajectories, execution errors, and verifier feedback are distilled into Agent~Skills and committed only after validation under a graph-complexity prior.

% \textbf{Contributions.}
% This work makes three contributions.
% First, we formulate workflow-based image creation as a skill-augmented MDP over executable graph edits, runtime feedback, verifier feedback, and reusable skills, making harness and skill design choices empirically testable.
% Second, we introduce \ours{}, a harness for unmodified ComfyUI that combines typed graph editing, stage-gated tool access, rollback repair, region-level VLM verification, episodic memory, and progressive-disclosure skill loading.
% Third, we propose a self-evolving skill-management procedure that converts trajectories and verifier feedback into held-out-validated Agent~Skills under a graph-complexity prior. Across four benchmark splits, two image backbones, and three agent models, \ours{} obtains the highest average score across six agent--backbone configurations; with Qwen-3.6-35B-A3B controlling LongCat-Image, it improves the average score from $61.09$ for a verifier-only \comfygems{}-style baseline to $76.34$. The skill evolver produces $318$ unique skills that account for roughly $50\%$ of subsequent skill invocations, and human ratings on $2{,}400$ images corroborate the same trend.

% Our contributions include:
% \begin{itemize}[leftmargin=*]
%     \item  We formulate workflow-based image creation as a skill-augmented MDP over executable graph edits, runtime feedback, verifier feedback, and reusable skills, making harness design and skill reuse explicit parts of the control problem.
%     \item  We introduce \ours{}, an agentic harness for an \emph{unmodified} ComfyUI runtime that combines typed graph editing, stage-gated tool access, rollback repair, region-level VLM verification, episodic memory, and progressive-disclosure skill loading.
%     \item  We propose a held-out-validated skill-evolution procedure that converts trajectories, execution errors, and verifier feedback into Agent~Skills under a graph-complexity prior. Across four benchmark splits, two image backbones, and three agent models, \ours{} obtains the best average score, and its $318$ evolved skills account for roughly $50\%$ of later skill invocations.
% \end{itemize}

\section{Introduction}
\label{sec:introduction}

% Modern generative systems are moving from prompt-only interfaces~\cite{cao2025controllable} toward executable \emph{agentic workflow control}~\cite{xu2025comfyui}. 
% while prompt-only interfaces are easy to use, but provide limited control over intermediate components, hyperparameters, and failure repair~\cite{cao2025controllable}, Workflow-based systems such as ComfyUI expose generation as an editable
% pipeline, enabling users to inspect and modify text encoders, conditioning,
% sampling, refinement, regional editing, and inpainting
% steps~\cite{gal2024comfygen,huang2025comfygpt}.
% This makes generation more inspectable and repairable, but also shifts the burden from prompt writing to procedure construction.

% Modern generative systems are moving beyond prompt-only interfaces toward executable workflow control~\cite{cao2025controllable,xu2025comfyui}. 
% Prompting is easy to use, but hides many of the decisions that determine the final image: how conditioning is applied, how samples are refined, where regional edits are made, and when inpainting or other repair steps are needed. 
% Workflow systems such as ComfyUI~\cite{comfyui_registry} make these decisions explicit by exposing generation as an editable pipeline~\cite{gal2024comfygen,huang2025comfygpt}. 
% The benefit is control and inspectability; the cost is that users and agents must now construct, debug, and adapt a valid procedure rather than simply write a better prompt.
% %
% This flexibility comes with a cost: effective workflow construction requires procedural knowledge about component compatibility, model constraints, visual failure localization, and graph repair, motivating agents that can build, refine, and repair workflows automatically~\cite{gal2024comfygen,sobania2024comfygi}.

Modern generative agents are moving beyond prompt-only chat interfaces toward
executable workflow control~\cite{cao2025controllable,xu2025comfyui}.
%
In image generation, this shift is especially important because prompt-only interfaces hide many decisions that shape the final image, such as how conditioning is applied, how the workflow is executed, and how failures are detected and repaired.
% how samples are refined, where regional edits are made, and when inpainting or other repair steps are needed. 
Workflow systems such as ComfyUI~\cite{comfyui_registry} expose these decisions as an editable pipeline, making generation inspectable, controllable, and reusable~\cite{gal2024comfygen,huang2025comfygpt}. 
%
The same flexibility, however, turns image creation into a procedural control problem: a user or agent must choose compatible components, respect model constraints, localize visual failures, and repair the graph without breaking execution. 
This motivates workflow agents that can automatically build, refine, and repair executable generation pipelines~\cite{gal2024comfygen,sobania2024comfygi}.

% \emph{agentic workflow control} is useful across many everyday tasks, and visual
% generation is a representative case where agents must control complex image and video pipelines~\cite{xu2025comfyui}.
% %
% Prompt-only interfaces are easy to use, but provide limited control over
% intermediate components, hyperparameters, and failure repair~\cite{cao2025controllable}.
% %
% Workflow-based systems such as ComfyUI expose generation as an editable
% pipeline, enabling users to inspect and modify text encoders, conditioning,
% sampling, refinement, regional editing, and inpainting
% steps~\cite{gal2024comfygen,huang2025comfygpt}.
% %
% ComfyUI's large open-source ecosystem, including over 100K GitHub stars and
% 800+ custom-node authors, shows strong demand for controllable creative
% workflows~\cite{comfyui_registry}.
% %
% However, this flexibility also makes workflow construction difficult for beginners, motivating agents that can automatically build, refine, and repair workflows to help users learn these tools and automate complex generation tasks~\cite{gal2024comfygen,sobania2024comfygi}.


% Language-model agents are moving from answering questions to controlling executable workflows. In \emph{agentic workflow control}, an agent must select tools, update external state, interpret execution failures, judge partial outputs, and reuse experience from prior attempts~\cite{wang2023voyager,wu2024copilot,xie2024osworld,workarena2024,chezelles2025browsergym,xu2025agents,wu2026saber}.  
% %
% This shift is promising because workflows expose expert procedures as inspectable, repeatable traces rather than one-off outputs~\cite{gal2024comfygen}. 
% %
% However, workflow control is much harder than answer generation: the agent must choose valid actions, update external state, interpret runtime feedback, and recover from failures over a long horizon. 
% %
% A single invalid operation can break the workflow, and the error is often only visible after execution~\cite{su2026comfysearch}.

% Recent workflow-generation agents~\cite{wang2023voyager,wu2024copilot,xie2024osworld,workarena2024,chezelles2025browsergym,xu2025agents,gal2024comfygen} reduce this burden by translating natural language into executable graphs or refining workflows through feedback. 
% Yet most systems still treat the control interface and skill library as fixed components. 
% As a result, an agent may repair a bad layout, invalid node, or missing refinement stage during one run, but the fix is not necessarily validated, stored, and reused in later workflows.


% In \emph{agentic workflow control}, agents operate on expert procedures as
% inspectable, repeatable traces rather than producing one-off
% outputs~\cite{wang2023voyager,wu2024copilot,xie2024osworld,workarena2024,chezelles2025browsergym,xu2025agents,gal2024comfygen}.
% %
% This is challenging because agents must interact with an execution environment through a harness, where one invalid action can break the workflow and errors may appear only after execution~\cite{pan2026natural,su2026comfysearch}.
% %
% Existing workflow-generation agents reduce this burden by generating or
% refining graphs from natural language~\cite{xu2025comfyui,jiang2026genagent,xue2025comfybench}, while systems such as GEMS show that closed-loop refinement,
% memory, and skills can improve multimodal generation~\cite{he2026gems}.
% %
% However, these systems often treat the interface and skill library as static or passively accumulated components.
% %
% Thus, repeated failures may be repaired locally during a run, but without a
% mechanism for validating and storing these fixes as reusable skills, they cannot be systematically reused in later tasks~\cite{wang2023voyager}.


Workflow agents therefore face a different problem from prompt-only generation: they must control an executable procedure, not just produce a final artifact.
%
Each step is mediated by a harness that exposes graph edits, runtime feedback, and recovery mechanisms; one invalid operation can break execution, and some failures are only revealed after the workflow is run~\cite{wang2023voyager,wu2024copilot,xie2024osworld,workarena2024,chezelles2025browsergym,xu2025agents,gal2024comfygen,pan2026natural,su2026comfysearch}.
%
Recent workflow-generation agents reduce this burden by generating or refining graphs from natural language~\cite{xu2025comfyui,jiang2026genagent,xue2025comfybench}, while systems such as GEMS show the value of closed-loop refinement, memory, and skills for multimodal generation~\cite{he2026gems}.
%
However, their control interfaces and skill libraries are usually fixed, or expanded passively from experience.
%
Thus, a repair that succeeds in one run rarely becomes a validated procedure that can be invoked safely in future workflows~\cite{wang2023voyager}.

% Image creation provides a concrete instance of this control problem. 
% %
% Prompt-only generation is easy to use, but offers little structure for controlling intermediate decisions or repairing failures~\cite{cao2025controllable}. 
% %
% Workflow-based generation instead exposes the generation process as an editable pipeline, where choices such as conditioning, sampling, refinement, regional editing, and inpainting can be inspected and modified~\cite{gal2024comfygen,huang2025comfygpt}. 
% %
% This interface makes generation more controllable, but shifts the burden from prompt writing to procedure construction: the agent must choose compatible components, respect model constraints, localize visual failures, and repair the graph without breaking execution. 
% %
% Existing workflow-generation agents reduce this burden by producing or refining graphs from natural language~\cite{xu2025comfyui,jiang2026genagent,xue2025comfybench}; systems such as GEMS further show that closed-loop refinement, memory, and skills can improve multimodal generation~\citep{he2026gems}. 
% However, these systems still largely treat the control interface and skill library as fixed or accumulated components, rather than testable parts of the workflow-control system. 
% As a result, repeated failures are repaired locally instead of becoming validated procedures that can be reused in later tasks.

% Reliable workflow control requires two coupled forms of infrastructure. 
% A harness makes edits executable: it exposes typed actions, validates graph changes, surfaces runtime errors, and supports rollback. 
% A skill library makes experience reusable: it stores procedures that helped solve previous workflow failures. 
% Either component alone is insufficient. A harness without evolving skills repeatedly rediscovers similar repairs; skills without a disciplined harness become brittle text recipes that may be mis-triggered or invalid for the current graph.

% Recent work has shown growing interest in agent harnesses~\cite{lou2026autoharness}, memory systems~\cite{xu2025mem, zhang2026memrl},
% skill management~\cite{xia2026skillrl,yu2025polyskill}, and self-evolving agents~\cite{wu2026coevolvingllmdecisionskill} for workflow control.
% %
% These systems enable agents to execute commands, use tools, control workflows,
% and complete complex tasks by accumulating reusable experience.
% %
% General-purpose agent frameworks such as OpenClaw~\cite{openclaw2026} and
% Hermes-Agent~\cite{nousresearch2026hermesagent}, as well as automated research
% systems such as AutoResearch~\cite{karpathy2026autoresearch}, illustrate how
% memory and skills can support long-horizon workflow execution.
% %
% A parallel line of work studies self-evolving agents that improve through
% trial and error by interacting with an environment, receiving feedback, and
% updating their behavior from accumulated experience~\cite{wu2025evolver,xiang2026systematic,huang2025r,zhang2026memskill,he2026active}.
% %
% For image-generation workflow control, however, neither an agent harness nor
% static skill management is sufficient on its own.
% %
% A harness makes each workflow edit executable, observable, and recoverable,
% while skill management preserves useful procedures across tasks.
% %
% Without a disciplined harness, skills can become brittle text instructions that
% are mis-triggered, invalid for the current graph, or unnecessarily complex.
% %
% Without evolving skills, successful repairs remain local to a single run and do
% not improve future workflow construction.
% %
% Thus, the central challenge is not only to refine a workflow during one run,
% but also to use verifier feedback from that run to improve future control.

% This limitation suggests that workflow agents need infrastructure for both controlling the current executable state and carrying useful experience across tasks.
% Turning one-off repairs into reusable workflow competence requires two pieces of infrastructure.
% The first is a \emph{harness}: the external structure that exposes tools, memory, feedback, and state transitions to an otherwise general model
% \cite{madaan2023self,shinn2023reflexion,young2025effective,lou2026autoharness,lee2026meta,xu2026agent}.
% The second is \emph{skill management}: the mechanism that turns repeated trajectories into reusable procedural knowledge
% \cite{wang2023voyager,wu2025evolver,xia2026skillrl,ni2026trace2skill,zhai2025agentevolver,gao2025survey,fang2025comprehensive}.
% % In workflow control, these two components must be coupled rather than treated as independent add-ons.
% % A harness without evolving skills can repair the current workflow but repeatedly rediscovers similar fixes; skills without a disciplined harness can become brittle instructions that are mis-triggered, invalid for the current graph, or unnecessarily complex.
% % This motivates our central question:  \emph{how can verifier feedback support both immediate workflow repair and the long-term evolution of a reusable skill library?}
% %
% For workflow control, neither component is sufficient on its own. 
% A harness can make each edit executable and recoverable, but without evolving skills it only repairs the current workflow and repeatedly rediscovers similar fixes. 
% Skill management can preserve useful procedures across tasks, but without a disciplined harness those procedures become brittle text instructions that may be mis-triggered, invalid for the current graph, or unnecessarily complex. 
% Thus, the central challenge is not only to refine a workflow during one run, but to use feedback from that run to improve future control. 
% This motivates our question: 
% %
% % \emph{how can verifier feedback support both immediate workflow repair and the long-term evolution of a reusable skill library?}
% %
% \emph{can verifier feedback support both immediate
% workflow repair and the long-term evolution of a reusable skill library?}

This limitation suggests that workflow agents need infrastructure for both controlling the current executable state and carrying useful experience across tasks.
%
Turning one-off repairs into reusable workflow competence requires two coupled components: a \emph{harness}, which exposes tools, feedback, memory, and state transitions to an otherwise general model~\cite{madaan2023self,shinn2023reflexion,young2025effective,lou2026autoharness,lee2026meta,xu2026agent}, and \emph{skill management}, which converts repeated trajectories into reusable procedural knowledge~\cite{wang2023voyager,wu2025evolver,xia2026skillrl,ni2026trace2skill,zhai2025agentevolver,gao2025survey,fang2025comprehensive}.
%
Neither is sufficient on its own.
%
A harness without evolving skills repeatedly rediscovers similar repairs, while skills without a disciplined harness can become brittle instructions that are mis-triggered, invalid for the current graph, or unnecessarily complex.
%
Thus, the challenge is not only to refine a workflow during one run, but to turn feedback from that run into reusable control knowledge.
%
This motivates our question: \emph{can verifier feedback support both immediate workflow repair and the long-term evolution of a reusable skill library?}

% This motivates our question: \emph{can verifier feedback support both immediate
% workflow repair and the long-term evolution of a reusable skill library?}
% %
% Inspired by agentic workflow control and self-evolution, we propose \ours{}, a
% self-evolving framework for controlling image-generation workflows.
% %
% \ours{} integrates three components.
% %
% First, a harness represents workflow construction as typed graph edits, exposes
% tools through a stage-gated router, and uses rollback to recover from invalid
% edits~\cite{madaan2023self,shinn2023reflexion,young2025effective,lou2026autoharness,lee2026meta,xu2026agent}.
% %
% Second, a region-level VLM verifier converts visual failures into localized
% repair suggestions, allowing the agent to refine workflows using both verifier
% and runtime feedback.
% %
% Third, a progressively disclosed skill library converts successful
% trajectories, execution errors, and verifier feedback into reusable
% Agent~Skills, which are committed only after validation under a
% graph-complexity prior~\cite{wang2023voyager,wu2025evolver,xia2026skillrl,ni2026trace2skill,zhai2025agentevolver,gao2025survey,fang2025comprehensive}.


% This motivates our question: \emph{can verifier feedback support both immediate workflow repair and the long-term evolution of a reusable skill library?}
% We study this question in ComfyUI workflow synthesis, where workflow repair and skill evolution can be evaluated beyond the final image.
% Each workflow is an executable graph: invalid edits are rejected by the runtime, rendered images can be checked against decomposed visual requirements, and candidate skills can be tested on held-out prompts before entering the library.
% We introduce \ours{}, an agentic harness around an \emph{unmodified} ComfyUI runtime.
% \ours{} casts workflow construction as typed graph editing, gates tool access by construction stage, and uses rollback to recover from invalid edits~\cite{madaan2023self,shinn2023reflexion,young2025effective,lou2026autoharness,lee2026meta,xu2026agent}.
% A region-level VLM verifier then converts visual failures into localized repair suggestions, enabling refinement from both runtime and verifier feedback.
% Finally, \ours{} maintains a progressively disclosed skill library that distills successful trajectories, execution errors, and verifier feedback into reusable Agent~Skills, committing updates only after validation under a graph-complexity prior~\cite{wang2023voyager,wu2025evolver,xia2026skillrl,ni2026trace2skill,zhai2025agentevolver,gao2025survey,fang2025comprehensive}.

% To study workflow repair and skill evolution together, we need a setting where an agent's decisions can be evaluated beyond the final output. ComfyUI workflow synthesis provides such a setting: each workflow is an executable graph, so invalid edits are rejected by the runtime, rendered images can be checked against decomposed visual requirements, and candidate skills can be tested on held-out prompts before entering the library.

% This motivates our question: \emph{Can verifier feedback support both immediate workflow repair and the long-term evolution of a reusable skill library?}
%
% We study this question in ComfyUI workflow synthesis, where workflow repair and skill evolution can be evaluated beyond the final image.
% Each workflow is an executable graph: invalid edits are rejected by the runtime, rendered images can be checked against decomposed visual requirements, and candidate skills can be tested on held-out prompts before entering the library.
%
Inspired by agentic workflow control and self-evolution~\cite{wu2025evolver, zhai2025agentevolver}, we propose \ours{}, a self-evolving framework for controlling image-generation workflows.
%
\ours{} represents workflow construction as typed graph edits over an \emph{unmodified} ComfyUI runtime.
A stage-gated router exposes tools safely, rollback recovers from invalid edits, and a region-level vision-language model (VLM) verifier converts visual failures into localized repair suggestions.
Successful trajectories, execution errors, and verifier feedback are then distilled into progressively disclosed Agent~Skills, which are committed only after held-out validation under a graph-complexity prior.

% \textbf{Contributions.}
% This work makes three contributions.
% First, we formulate workflow-based image creation as a skill-augmented MDP over executable graph edits, runtime feedback, verifier feedback, and reusable skills, making harness and skill design choices empirically testable.
% Second, we introduce \ours{}, a harness for unmodified ComfyUI that combines typed graph editing, stage-gated tool access, rollback repair, region-level VLM verification, episodic memory, and progressive-disclosure skill loading.
% Third, we propose a self-evolving skill-management procedure that converts trajectories and verifier feedback into held-out-validated Agent~Skills under a graph-complexity prior. Across four benchmark splits, two image backbones, and three agent models, \ours{} obtains the highest average score across six agent--backbone configurations; with Qwen-3.6-35B-A3B controlling LongCat-Image, it improves the average score from $61.09$ for a verifier-only \comfygems{}-style baseline to $76.34$. The skill evolver produces $318$ unique skills that account for roughly $50\%$ of subsequent skill invocations, and human ratings on $2{,}400$ images corroborate the same trend.

% Our contributions include:
% \begin{itemize}[leftmargin=*]
%     \item  We formulate workflow-based image creation as a skill-augmented MDP over executable graph edits, runtime feedback, verifier feedback, and reusable skills, making harness design and skill reuse explicit parts of the control problem.
%     \item  We introduce \ours{}, an agentic harness for an \emph{unmodified} ComfyUI runtime that combines typed graph editing, stage-gated tool access, rollback repair, region-level VLM verification, episodic memory, and progressive-disclosure skill loading.
%     We propose a held-out-validated skill-evolution procedure that converts trajectories, execution errors, and verifier feedback into Agent~Skills under a graph-complexity prior. 
%     \item   Across four benchmark splits, two image backbones, and three agent models, \ours{} obtains the best average score, and its $318$ evolved skills account for roughly $50\%$ of later skill invocations.
%     We evaluate \ours{} with three agents, Claude-Sonnet-4.5~\cite{anthropic2025claude}, Gemma-4-E4B-it~\cite{gemma4_2026}, and Qwen-3.6-35B-A3B~\cite{qwen3}, on two image-generation models, LongCat-Image~\cite{team2025longcat} and Z-Image-Turbo~\cite{zimage2025}. 
% % 
% Across these settings, \ours{} outperforms agent harness workflow control without skill evolution by an average of 4 points out of 100, and outperforms agent workflow control without refinement by 10 points. 
% % 
% We further conduct user annotation on 2{,}400 randomly selected images, where users prefer \ours{} over both ablations on average.
% \end{itemize}

Our contributions include:
\begin{itemize}[leftmargin=*]
    \item 
    We formulate workflow-based image creation as a skill-augmented Markov Decision Process over executable graph edits, runtime feedback, verifier feedback, and reusable skills, making harness design and skill reuse explicit parts of the control problem.

    % \item
    % We introduce \ours{}, an agentic harness for an \emph{unmodified} ComfyUI runtime. \ours{} combines typed graph editing, stage-gated tool access, rollback repair, region-level VLM verification, episodic memory, and progressive-disclosure skill loading. It further includes a held-out-validated skill-evolution procedure that converts trajectories, execution errors, and verifier feedback into Agent~Skills under a graph-complexity prior.

   \item We introduce \ours{}, an agentic harness for an \emph{unmodified} ComfyUI runtime.
    %
    \ours{} combines typed graph editing for workflow construction, VLM-based
    feedback for workflow refinement, and a skill-evolution loop that proposes,
    validates, and commits reusable Agent~Skills.
    %
    % These skills are distilled from trajectories, execution errors, and verifier
    % feedback, and are accepted only after held-out validation under a
    % graph-complexity prior.

     \item We evaluate \ours{} across four benchmark splits, two image backbones, and three agent models. \ours{} achieves the best average score, improves over harness-only control by 4 points and no-refinement control by 10 points, is preferred by human annotators on 2{,}400 images, and uses $318$ evolved skills for roughly $50\%$ of later skill invocations.
    % \item 
    % We evaluate \ours{} across four benchmark splits, two image-generation backbones, LongCat-Image~\cite{team2025longcat} and Z-Image-Turbo~\cite{zimage2025}, and three workflow-control agents, Claude-Sonnet-4.5~\cite{anthropic2025claude}, Gemma-4-E4B-it~\cite{gemma4_2026}, and Qwen-3.6-35B-A3B~\cite{qwen3}. \ours{} obtains the best average score, improves over harness-only control by 4 points and no-refinement control by 10 points, and is preferred by human annotators on 2{,}400 images. Its $318$ evolved skills account for roughly $50\%$ of later skill invocations, showing that the system accumulates reusable workflow knowledge rather than only repairing individual runs.
\end{itemize}

\section{Related Work}

% \wxy{why list these tools, can we use cites?}

% \subsection{Workflow-based content creation and agentic control}
% %
% Node-based, workflow-oriented content creation is a long-standing paradigm in creative software. Systems such as Blender’s geometry and shader nodes~\cite{blender}, Houdini’s procedural networks~\cite{houdini}, Nuke’s compositor~\cite{nuke}, Unreal Engine Blueprints~\cite{unrealengine} all share a common principle: the workflow graph itself is the artifact, making the creative process modular, inspectable, and reusable.
% %
% %
% ComfyUI~\cite{comfyanonymous2023comfyui} brings this paradigm to diffusion-based generation and has become one of the most widely used open-source tools for assembling image, video, and audio-visual generation pipelines~\cite{xu2025comfyui,guo2025comfymind}.
% %
% Such workflow-based tools offer important benefits for creators, especially those without programming experience or direct access to local compute resources such as GPUs~\cite{angert2023spellburst,tamilselvam2019visual,vuruma2024cloud}.
% %
% However, they remain difficult to learn in practice: documentation is often long and fragmented, and there are few structured courses or systematic tutorials for new users~\cite{huang2025comfygpt, guo2025comfymind}.
% %
% %
% A recent line of work treats ComfyUI as an \emph{agent target}. ComfyGen~\cite{gal2024comfygen} adaptively selects workflows from prompts; ComfyGPT~\cite{huang2025comfygpt} and GenAgent~\cite{jiang2026genagent} generate workflow graphs or code end-to-end through multi-agent collaboration; ComfyUI-R1~\cite{xu2025comfyui} introduces RL-tuned reasoning; and ComfyBench~\cite{xue2025comfybench} provides an evaluation benchmark.
% %
% These works aim to help creators get started more quickly and improve workflow efficiency. 
% %
% However, they focus on workflow generation as a one-shot output that is executed once. 
% %
% In contrast, we model workflow construction as a process in which the agent can iteratively refine graphs, accumulate experience over time, and improve future generations through reusable skills.
%

% In contrast, we formulate workflow construction as an iterative graph-editing process in a closed loop with a region-level VLM verifier. This enables the agent to progressively improve the workflow topology across attempts for a given prompt.
% %
% Beyond per-prompt refinement, our self-evolving skill management stores past successes and failures as reusable experience, while skill routing retrieves the most relevant prior skills to guide future workflow construction.

% \wxy{this is good, may shirnk a bit}

% \subsection{Workflow-based content creation and agentic control}

% Workflow graphs are a common interface for creative software, from Blender nodes~\cite{blender} and Houdini networks~\cite{houdini} to Nuke compositing~\cite{nuke} and Unreal Blueprints~\cite{unrealengine}. Their main advantage is that the graph itself is the artifact: it exposes intermediate structure, supports reuse, and makes complex pipelines easier to inspect than monolithic code. ComfyUI~\cite{comfyanonymous2023comfyui} brings this paradigm to diffusion-based generation, where users compose image, video, and audio-visual pipelines from node graphs~\cite{xu2025comfyui,guo2025comfymind}. While this lowers the barrier to building generative workflows, it also introduces a new usability problem: effective use still requires knowledge of node compatibility, model constraints, and scattered community recipes, which remain difficult for non-expert users to acquire~\cite{angert2023spellburst,tamilselvam2019visual,vuruma2024cloud,huang2025comfygpt,guo2025comfymind}. Recent work therefore treats ComfyUI as an agent-control target. ComfyGen~\cite{gal2024comfygen} selects workflows from prompts, ComfyGPT~\cite{huang2025comfygpt} and GenAgent~\cite{jiang2026genagent} synthesize workflow graphs or code with multi-agent collaboration, ComfyUI-R1~\cite{xu2025comfyui} studies RL-tuned reasoning, and ComfyBench~\cite{xue2025comfybench} provides an evaluation setting. These systems mainly frame the problem as workflow generation or refinement for the current prompt. Our work instead treats workflow construction as closed-loop agent control: COMFYCLAW edits executable graphs through a typed, stage-gated harness, repairs failures using localized verifier feedback, and evolves reusable skills that are admitted only after held-out validation under a graph-complexity prior.

% \subsection{Workflow-based content creation and agentic control}

% \subsection{Workflow graphs as controllable creative artifacts}


% \textbf{Workflow graphs as controllable creative artifacts.}
% %
% Workflow graphs are a standard interface in creative software, from Blender nodes~\cite{blender} and Houdini networks~\cite{houdini} to Nuke compositing~\cite{nuke} and Unreal Blueprints~\cite{unrealengine}. In these systems, the graph is the artifact: it exposes intermediate structure, supports reuse, and makes complex pipelines easier to inspect than monolithic code. ComfyUI~\cite{comfyanonymous2023comfyui} brings this paradigm to diffusion-based generation, where users compose image, video, and audio-visual pipelines from node graphs~\cite{xu2025comfyui,guo2025comfymind}. Although this interface lowers the barrier to generative workflows, effective use still requires knowledge of node compatibility, model constraints, and scattered community recipes~\cite{angert2023spellburst,tamilselvam2019visual,vuruma2024cloud,huang2025comfygpt,guo2025comfymind}. Recent work therefore treats ComfyUI as an agent-control target: ComfyGen~\cite{gal2024comfygen} selects workflows from prompts, ComfyGPT~\cite{huang2025comfygpt} and GenAgent~\cite{jiang2026genagent} synthesize graphs or code with multi-agent collaboration, ComfyUI-R1~\cite{xu2025comfyui} studies RL-tuned reasoning, and ComfyBench~\cite{xue2025comfybench} provides an evaluation setting. These systems mainly frame the task as workflow generation or refinement for the current prompt. In contrast, \ours{} treats workflow construction as closed-loop agent control: it edits executable graphs through a typed, stage-gated harness, repairs failures with localized verifier feedback, and promotes reusable skills only after held-out validation under a graph-complexity prior.

\textbf{Workflow graphs as controllable creative artifacts.}
%
Workflow graphs are common in creative software, from Blender nodes~\cite{blender} and Houdini networks~\cite{houdini} to Nuke compositing~\cite{nuke} and Unreal Blueprints~\cite{unrealengine}. In these systems, the graph is the artifact: it exposes intermediate structure, supports reuse, and makes complex pipelines easier to inspect than monolithic code. ComfyUI~\cite{comfyanonymous2023comfyui} brings the same idea to diffusion-based generation, where users build image, video, and audio-visual pipelines from node graphs~\cite{xu2025comfyui,guo2025comfymind}. While effective use still depends on node compatibility, model constraints, and scattered community recipes~\cite{angert2023spellburst,tamilselvam2019visual,vuruma2024cloud,huang2025comfygpt,guo2025comfymind}. Recent work therefore treats ComfyUI as an agent-control target: ComfyGen~\cite{gal2024comfygen} selects workflows from prompts, ComfyGPT~\cite{huang2025comfygpt} and GenAgent~\cite{jiang2026genagent} synthesize graphs or code through multi-agent collaboration, ComfyUI-R1~\cite{xu2025comfyui} studies RL-tuned reasoning, and ComfyBench~\cite{xue2025comfybench} provides an evaluation setting. These systems mostly optimize workflow generation or refinement for a single prompt. In contrast, \ours{} treats workflow construction as closed-loop control: it edits executable graphs through a typed, stage-gated harness, repairs failures with localized verifier feedback, and promotes reusable skills only after held-out validation under a graph-complexity prior.



% \subsection{Foundations of agent harnesses and skill usage}
% Agent skills and harness are important for workflow running and integration for application and tool usage. 
% %
% Voyager~\cite{wang2023voyager} establishes the now-standard agentic pattern:
% an LLM agent with an automatic curriculum, an executable skill library, and
% an iterative self-verification loop. 
% %
% Subsequent work refine the
% self-improvement signal.
% %
% Eureka~\cite{ma2023eureka} for reward design,
% Self-Refine~\cite{madaan2023self} and Reflexion~\cite{shinn2023reflexion} for prompt-level
% critique, OS-Copilot~\cite{wu2024copilot} for desktop tasks, and DSPy~\cite{khattab2023dspy}
% for declarative pipeline compilation. 
% %
% In parallel, the \textit{Anthropic Agent Skills}~\cite{agentskills2026specification}
% specification has standardised a `SKILL.md' package format with three-level progressive disclosure that has been adopted by Claude Code~\cite{anthropic2025claudecode},
% Hermes Agent~\cite{nousresearch2026hermesagent} and OpenClaw~\cite{openclaw2026},
% among others. 
% %
% \ours{} conforms to this spec and contributes (i) a
% domain-specific instantiation for image-generation workflow synthesis, (ii) a
% held-out-validated skill-mutation procedure with a complexity prior, and (iii)
% a stage-gated tool router that reduces hallucinated tool calls.

% SkillRL~\cite{xia2026skillrl} moves beyond raw trajectory memory by distilling experience into a hierarchical SkillBank and co-evolving the skill library with the policy through recursive skill-augmented reinforcement learning.

% EvoSkill~\cite{alzubi2026evoskill} discovers and refines reusable agent skills from execution failures, materializing them into structured skill folders and retaining only skills that improve held-out validation performance under a frozen base model.

% COS-PLAY~\cite{wu2026coevolvingllmdecisionskill} introduces a co-evolution framework where a decision agent learns to use reusable skills for long-horizon game playing, while a skill-bank agent continually discovers, refines, and updates those skills from unlabeled rollouts, enabling both the policy and skill library to improve together.


% \subsection{Foundations of agent harnesses and skill usage}

% \textbf{Harnessed agents with reusable skills.}
% %
% Recent agent systems increasingly use explicit skills, tool interfaces, and runtime harnesses to make long-horizon execution more reliable. Voyager~\cite{wang2023voyager} introduced a common template: a Large Language Model (LLM) agent improves through an automatic curriculum, an executable skill library, and iterative self-verification. Later work refined parts of this loop, including reward design in Eureka~\cite{ma2023eureka}, prompt-level critique in Self-Refine~\cite{madaan2023self} and Reflexion~\cite{shinn2023reflexion}, desktop-task scaffolding in OS-Copilot~\cite{wu2024copilot}, and declarative pipeline construction in DSPy~\cite{khattab2023dspy}. A parallel line treats skills as reusable agent artifacts. The \textit{Anthropic Agent Skills} specification~\cite{agentskills2026specification} defines a lightweight \texttt{SKILL.md} format with progressive disclosure, adopted by systems such as Claude Code~\cite{anthropic2025claudecode}, Hermes Agent~\cite{nousresearch2026hermesagent}, and OpenClaw~\cite{openclaw2026}. SkillRL~\cite{xia2026skillrl} distills experience into a hierarchical SkillBank and trains policies with recursively reused skills, EvoSkill~\cite{alzubi2026evoskill} mines and repairs skills from execution failures under held-out validation, and COS-PLAY~\cite{wu2026coevolvingllmdecisionskill} co-evolves a decision agent and skill-bank agent from unlabeled rollouts for long-horizon game play. 
% %
% % Our work builds on these ideas but targets harnessed, validated skill usage for image-generation workflow synthesis: we instantiate skills in a domain-specific tool workflow setting, mutate skills under held-out validation with a complexity prior, and use a stage-gated router to reduce hallucinated tool calls.
% %
% Our work extends self-evolving workflow control with skills: \ours{} combines typed, stage-gated graph editing with localized verifier feedback and held-out validation for skill mutation, enabling workflow skills to be learned, tested, and reused rather than manually authored or statically retrieved.

\textbf{Harnessed agents with reusable skills.}
%
Recent agent systems use explicit skills, tool interfaces, and runtime harnesses to make long-horizon execution more reliable. Voyager~\cite{wang2023voyager} set an influential template, where an LLM agent improves through an automatic curriculum, executable skill library, and iterative self-verification. Later work developed related pieces, including reward design in Eureka~\cite{ma2023eureka}, critique and reflection in Self-Refine~\cite{madaan2023self} and Reflexion~\cite{shinn2023reflexion}, desktop-task scaffolding in OS-Copilot~\cite{wu2024copilot}, and declarative pipeline construction in DSPy~\cite{khattab2023dspy}. A parallel line treats skills as reusable agent artifacts. The \textit{Anthropic Agent Skills} specification~\cite{agentskills2026specification} defines a lightweight \texttt{SKILL.md} format with progressive disclosure, used by systems such as Claude Code~\cite{anthropic2025claudecode}, Hermes Agent~\cite{nousresearch2026hermesagent}, and OpenClaw~\cite{openclaw2026}. Recent methods also learn or revise skills from experience: SkillRL~\cite{xia2026skillrl} builds a hierarchical SkillBank, EvoSkill~\cite{alzubi2026evoskill} mines and repairs skills from failures with held-out validation, and COS-PLAY~\cite{wu2026coevolvingllmdecisionskill} co-evolves decision and skill-bank agents from unlabeled game rollouts.
%
\ours{} brings this idea to workflow control: it combines typed, stage-gated graph editing with localized verifier feedback and held-out validation, so workflow skills can be learned, tested, and reused rather than manually written or statically retrieved.

% \wxy{need a para to link to the main contribution}

% \subsection{Self-evolving agent systems and agents that work for humans}
% %
% A growing class of LLM-based agent systems is designed to take long-horizon actions on a user’s behalf.
% %
% Recent open-source systems illustrate the broader harness design space in which our work sits. DeerFlow 2.0~\cite{bytedance2025deerflow} is a LangGraph-based super-agent harness with sandboxed execution, persistent memory, sub-agent delegation, and extensible skills. 
% %
% OpenClaw~\cite{openclaw2026} is a multi-channel personal assistant built around a skill-based architecture. 
% %
% Hermes Agent~\cite{nousresearch2026hermesagent} is organized around reusable skills and emphasizes autonomous skill creation and self-improvement through experience. 
% %
% These systems also reflect a broader shift toward skill-centric agent design, including progressive-disclosure style skill specifications that allow agents to load only the instructions relevant to the current task.
% %
% %
% In parallel, a growing research literature studies skill accumulation as a learning objective for agents, including work such as XSkill~\cite{jiang2026xskill}, EvolveR~\cite{wu2025evolver}, and self-evolving agents~\cite{gao2025survey, fang2025comprehensive}.
% %
% \ours{} follows this general harness perspective, but specializes it to a single structured environment: the ComfyUI content creation workflow graph.
% %
% This specialization matters because the action space, verifier feedback, and the unit of skill accumulation are all grounded in a concrete generative pipeline, enabling skills to be learned, reused, and improved around workflow construction rather than around unconstrained general-purpose tasks.
% \wxy{link to teh main contribution}


% Odysseus~\cite{shi2026odysseusscalingvlms100} an open RL training framework that makes VLM agents stable and sample-efficient for long-horizon visual decision-making, achieving strong progress in Super Mario Land and improved in-game and cross-game generalization.


% AgentLab~\cite{schmidgall2025agent} A multi-agent research-assistant system that takes a human research idea and executes literature review, experimentation, code generation, and report writing, while allowing human feedback at each stage. Relevant for human-agent collaboration and agents as research/workflow assistants.

% \subsection{Self-evolving agent systems and agents that work for humans}


\textbf{Skill-centric agents and self-improving harnesses.}
%
LLM agents are increasingly designed to act on a user's behalf over long horizons, often through harnesses that combine tool use, memory, delegation, and reusable skills. Recent open-source systems illustrate this shift: DeerFlow 2.0~\cite{bytedance2025deerflow} uses a LangGraph-based harness with sandboxed execution, persistent memory, sub-agents, and extensible skills; OpenClaw~\cite{openclaw2026} builds a multi-channel assistant around skill-based operation; and Hermes Agent~\cite{nousresearch2026hermesagent} emphasizes reusable skills and autonomous skill creation. A related research line studies skill accumulation and self-improvement as learning objectives, including XSkill~\cite{jiang2026xskill}, EvolveR~\cite{wu2025evolver}, and broader surveys of self-evolving agents~\cite{gao2025survey,fang2025comprehensive}. Other systems target human-facing long-horizon work more directly: Odysseus~\cite{shi2026odysseusscalingvlms100} studies stable RL for vision-language models (VLM) agents in long-horizon visual control, while AgentLab~\cite{schmidgall2025agent} executes research workflows with human feedback. 
%
These systems show the promise of skill-centric agents, but their skills are often used in broad, open-ended settings where effectiveness and reuse are hard to evaluate. 
% Our work studies the same question in executable image-generation workflows: \ours{} turns workflow construction into closed-loop graph control, where verifier feedback supports local repair and reusable skills are promoted only after held-out validation under a graph-complexity prior.

\section{Method}
\label{sec:method}

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{figures/framework.pdf}
    \caption{\textbf{Overall framework of \ours{}.}
    The agent edits a ComfyUI workflow graph, the runtime renders a candidate image, the verifier returns requirement-level and region-level feedback, and the agent evolves skills that can be reused in future workflow-construction runs.}
    \label{fig:overview}
    \vspace{-10pt}
\end{figure}
% \wxy{we need to clarify the purpose of this section. what's this for, probelm setting or othrs, should we give some equations?}

% \ours{} is an agentic framework for workflow-based image generation with reusable workflow skills. The framework consists of three main parts: \emph{workflow synthesis}, \emph{verifier-guided refinement}, and \emph{skill evolution}. First, \ours{} treats image generation as \emph{workflow synthesis}. Given a prompt $p$, an LLM agent constructs a ComfyUI workflow graph through typed graph edits and submits it to the runtime for rendering. A \emph{VLM verifier} then evaluates the rendered image against the prompt and returns both a scalar reward and localized repair feedback. The agent uses this feedback, together with runtime errors, to refine the workflow over multiple iterations.
% Across prompts, recurring successes and failures are distilled into validated Agent Skills, which are stored in a skill library and retrieved in future runs. Figure~\ref{fig:overview} summarizes the pipeline.

\ours{} is an agentic framework for workflow-based image generation with reusable workflow skills. It has three components: \emph{workflow construction}, \emph{verifier-guided refinement}, and \emph{skill evolution}. 
%
Given a prompt $p$, an LLM agent constructs a ComfyUI workflow graph through typed edits and submits it to the runtime for rendering. 
%
A VLM verifier scores the image against the prompt and returns localized repair feedback. 
%
The agent uses this feedback, along with runtime errors, to refine the workflow over multiple iterations.
%
Across prompts, recurring successes and failures are distilled into validated Agent Skills, stored in a skill library, and retrieved in future runs.
%
Figure~\ref{fig:overview} summarizes the pipeline.

% \subsection{Method}
% \label{sec:method}
% In this section, we introduce our agent reused across runs and revised after completed workflow-refinement and skill evolution framework.
% %
% The framework consists of three main parts: workflow synthesis, verifier-guided refinement, and skill evolution.
% %
% First, \ours{} treats image generation as \emph{workflow synthesis}: given a prompt $p$, an LLM agent loads the necessary tools and retrieves relevant skills to edit a ComfyUI workflow graph $G$, which is then submitted to ComfyUI for rendering.
% %
% Second, the ComfyUI runtime produces a candidate image, and a Vision-Language Model (VLM) verifier evaluates the image against the prompt and returns structured feedback to guide the next graph edit.
% %
% Third, the agent uses VLM feedback and runtime errors from workflow construction to extract reusable experience, evolve new skills, and store them in the skill library for future prompts.
% %
% Figure~\ref{fig:overview} summarizes the overall \ours{} pipeline.

% % \subsection{Background}

% % \subsection{Preliminaries: Workflows and Agent Skills}


\subsection{Preliminaries: Workflows and Agent Skills}

% % In this section, we briefly go over the background knowledge for workflows and agent skills.

% \paragraph{ComfyUI workflow graphs.}
% A ComfyUI workflow is a directed acyclic graph $G=(V,E)$.
% Each node $v\in V$ represents an operation such as text encoding, latent
% sampling, LoRA loading, regional conditioning, upsampling, inpainting, or image
% decoding.
% Edges $E$ pass intermediate objects between nodes.
% Given a text prompt $p$, the ComfyUI runtime executes the graph and renders an
% image or video.
% %
% Unlike prompt-only image generation, workflow-based generation can improve an
% image by changing both the prompt text and the underlying graph structure.

% % \textbf{ComfyUI workflow graphs.}
% % We model a ComfyUI workflow as a directed graph $G=(V,E)$.
% %
% % %
% Each node $v \in V$ denotes an operation, such as text encoding, latent sampling, LoRA loading, regional conditioning, upsampling, inpainting, or image decoding.
% %
% % %
% Edges $E$ pass intermediate objects between operations.
% % Given a prompt $p$, the ComfyUI runtime executes the graph to produce an image or video.
% %
% % %
% Compared with prompt-only generation, workflow-based generation exposes a larger control space: the agent can modify both the prompt and the computation graph that realizes it.

\textbf{ComfyUI workflow graphs.}
We represent a ComfyUI workflow as a directed graph $G=(V,E)$.
Nodes $V$ define the operations in the generation pipeline, including text encoding, latent sampling, LoRA loading, regional conditioning, upsampling, inpainting, and image decoding.
Edges $E$ carry intermediate outputs from one operation to the next.
Given a prompt $p$, ComfyUI executes the graph to render an image or video.
This graph-based interface gives the agent more control than prompt-only generation, since it can revise both the prompt and the pipeline that processes it.


% \textbf{ComfyUI workflow graphs.}
% % We model a ComfyUI workflow as a directed graph $G=(V,E)$.
% % Each node $v \in V$ denotes an operation, such as text encoding, latent
% % sampling, LoRA loading, regional conditioning, upsampling, inpainting, or image
% % decoding.
% % Edges $E$ pass intermediate objects between operations.
% % Given a prompt $p$, the ComfyUI runtime executes the graph to produce an image
% % or video.
% % Compared with prompt-only generation, workflow-based generation exposes a larger
% % control space: the agent can modify both the prompt and the computation graph
% % that realizes it.


% % \paragraph{Workflow editing.}
% % A workflow composes of a sequence of typed graph edits.
% % %
% The agent may add or delete nodes such as connecting nodes, changing node parameters,
% % modifying prompts, inserting LoRA modules, adding regional attention, or introducing
% % refinement passes such as hires-fix and inpainting.
% % %
% The agent submits the constructed workflow to ComfyUI to render images.

% A submitted workflow must pass ComfyUI validation before it can be rendered.
% If validation fails, the runtime returns a structured error that the agent can
% use to repair the graph.

\textbf{Workflow editing.}
We treat workflow construction as a sequence of graph edits.
The agent can add or remove nodes, connect or disconnect edges, adjust node paramete workflow-constructed, it is submitted to ComfyUI for execution.

% \textbf{Agent skills.}
% Agent Skills are reusable procedures stored as \texttt{SKILL.md} files.
% Each skill contains a short description, optional triggers, and imperative
% workflow-editing instructions.
% To keep the context small, the agent initially sees only skill names and
% descriptions.
% The full skill body is loaded only when the agent explicitly calls
% \texttt{read\_skill} for a specific skill.
% %
% Skills act as reusable workflow-construction knowledge that can be
% retrieved during generation and updated after each agent completion of a workflow construction run.

\textbf{Agent skills.}
Agent skills are reusable procedures stored as \texttt{SKILL.md} files.
Each skill includes a short description, optional triggers, and step-by-stepstep-by-step instructions for editing a workflow graph for editing a workflow graph.
To keep the context small, the agent initially sees only the the skill names and descriptions.
It loads tIt loads the full skill only when it explicitly calls \texttt{read\_skill}.
In this way, skills provide retrievable workflow-editing knowledge that can be reused across runs and revised after completed workflow-editing attempts.


% \subsection{Method}
% \label{sec:method}
% In this section, we introduce our agent reused across runs and revised after completed workflow-refinement and skill evolution framework.
% %
% The framework consists of three main parts: workflow synthesis, verifier-guided refinement, and skill evolution.
% %
% First, \ours{} treats image generation as \emph{workflow synthesis}: given a prompt $p$, an LLM agent loads the necessary tools and retrieves relevant skills to edit a ComfyUI workflow graph $G$, which is then submitted to ComfyUI for rendering.
% %
% Second, the ComfyUI runtime produces a candidate image, and a Vision-Language Model (VLM) verifier evaluates the image against the prompt and returns structured feedback to guide the next graph edit.
% %
% Third, the agent uses VLM feedback and runtime errors from workflow construction to extract reusable experience, evolve new skills, and store them in the skill library for future prompts.
% %
% Figure~\ref{fig:overview} summarizes the overall \ours{} pipeline.




% \subsubsection{Workflow Construction}
\subsection{Workflow Construction}
\label{sec:method:workflow-construction}
%
For the first stage, given a prompt $p$, the agent enters the planning stage,
where it identifies the target image-generation model, reads relevant tools and
skills, and plans how to construct the workflow.
%
We represent the workflow as a directed acyclic graph (DAG)
% \begin{equation}
%     G_t = (V_t, E_t),
% \end{equation}
%
$G_t = (V_t, E_t)$
%
where $V_t$ denotes the set of workflow nodes and $E_t$ denotes the data-flow
edges at refinement step $t$.
%
The agent first builds an initial workflow $G_0$, a minimal \emph{spine} graph
that loads the diffusion model, encodes the prompt with a text encoder, samples
the latent representation, decodes the image, and saves the output.
%
This initial graph provides a valid starting point for later refinement.

The agent then edits the workflow through a sequence of graph actions:
\begin{equation}
    G_{t+1} = \mathrm{Edit}(G_t, a_t),
    \qquad a_t \in \mathcal{A},
\end{equation}
where $\mathcal{A}$ includes node insertion, node connection, parameter
updates, prompt edits, LoRA insertion, regional conditioning, and refinement
passes.
%
The goal of workflow construction is to find a final workflow $G_T$ that reaches the verifier reward threshold (Section~\ref{subsec:vlm-verifier}).

Skills are used throughout workflow construction but are exposed to the agent selectively through a trigger-based router.
%
Each skill $\sigma_i \in \skillset$ contains lightweight metadata, including a
name, short description, tags, and trigger phrases.
%
Given the current workflow stage and verifier feedback, the agent scores each skill by relevance to the skill description and trigger metadata. Only the top-$K$ skills are shown to the agent.
%
The full skill body is loaded only when the agent explicitly calls
\texttt{read\_skill} .
%
This progressive exposure keeps the context small while still allowing the agent to access detailed procedures for workflow construction and repair.

After the spine graph is created, the agent moves to the construction stage.
%
In this stage, it edits the workflow DAG by adding or connecting nodes, setting
parameters, and modifying the graph structure according to the prompt
requirements.
%
The agent then enters the enhancement stage, where it can apply higher-level
workflow changes such as adding LoRA modules, regional attention, mask-based
conditioning, or refinement passes.
%
Together, these three stages correspond to the planning, construction, and
enhancement blocks shown at the top of Figure~\ref{fig:overview}.

% The updated workflow is submitted to the ComfyUI runtime:
% \begin{equation}
%     y_t = \mathrm{ComfyUI}(G_t, p).
% \end{equation}
% %
% If $y_t$ is a runtime error, the error signal is sent back to the agent and the
% agent repairs the workflow before resubmitting it.
% %
% If $y_t$ is an image $x_t$, the VLM verifier evaluates the image against the
% prompt and returns a reward and feedback:
% \begin{equation}
%     r_t, f_t = V_{\phi}(x_t, p).
% \end{equation}
% %
% When $r_t$ is below the target threshold $\tau$, the feedback is routed back to
% the agent for another round of workflow editing.
% %
% When $r_t \ge \tau$, the image is accepted as the final output:
% \begin{equation}
%     x^\star = \mathrm{render}(G_t; p)
%     \quad \text{if} \quad r_t \ge \tau.
% \end{equation}



% \subsubsection{VLM Verifier Loop}

% \subsection{VLM Verifier Loop}

\subsection{Verifier-Guided Refinement}
\label{subsec:vlm-verifier}
After the agent submits $G_t$, ComfyUI renders an image $I_t$ which is
passed to a VLM verifier.
%
The verifier first decomposes $p$ into a checklist of observable binary requirements $Q=\{q_i\}$.
%
For each $q_i$ it returns a binary pass/fail label grounded in the
image, together with a short natural-language justification; in
addition it returns a holistic detail score $s_{\mathrm{det}}\!\in\![0,10]$
that captures overall fidelity, composition, and absence of visual artifacts.
The harness combines the two signals into the scalar reward of
Eq.\,\ref{eq:reward}.

\paragraph{Vision-Language Model (VLM) as a Verifier.}
We use the agent as verifier to evaluate whether a generated image satisfies the prompt.
%
The verifier decomposes the prompt into observable requirements
$Q=\{q_i\}$, such as object count, attribute binding, spatial relation, style,
and anatomy.
%
It returns requirement-level pass or fail labels, a holistic detail score, localized failure descriptions, and concrete suggestions for workflow edits.
%
The score used by the harness is
\begin{equation}
  r \;=\; 0.6\cdot\!\frac{|Q^{\mathrm{pass}}|}{|Q|}
        \;+\; 0.4\cdot\!\frac{s_{\mathrm{det}}}{10},
  \label{eq:reward}
\end{equation}
% \begin{equation}
%   r \;=\; w_{\mathrm{req}}\!\cdot\!\frac{|Q^{\mathrm{pass}}|}{|Q|}
%         \;+\; w_{\mathrm{det}}\!\cdot\!\frac{s_{\mathrm{det}}}{10}.
%   \label{eq:reward}
% \end{equation}
% We use $(w_{\mathrm{req}},w_{\mathrm{det}})=(0.6,0.4)$.
where $s_{\mathrm{det}}$ is an additional one-pass quality score, ranging from 1 to 10, that measures the overall image quality and its alignment with the prompt.


\paragraph{Workflow Refinement loop.}
The verifier emits three structured components that drive the next iteration: (i) the failing-requirement set
$Q\!\setminus\!Q^{\mathrm{pass}}$, (ii) localized natural-language
descriptions of what went wrong (e.g.\ \textit{the leftmost figure has three arms}), and (iii) concrete edit suggestions phrased in workflow terms (\textit{apply regional prompting to isolate the throwing arm}).
%
These pieces are appended to the agent's next-iteration context and also forwarded to the skill-evolution loop (\S\ref{sec:skill-evolution}).
%
The refinement loop terminates when $r$ exceeds a satisfaction threshold
$\tau_{\mathrm{stop}}$ or after $K$ iterations, whichever comes first;
the iteration with the highest $r$ is committed as the final output.


% \paragraph{Workflow Refinement loop.}
% If the VLM verifier reward $r_t$ at iteration $t$ does not meet a satisfaction
% threshold $\tau_{\mathrm{stop}}$ or a maximum refinement iteration step, our harness framework triggers a repair step.
% %
% Three structured artifacts are appended to the agent's next-turn context:
% (i) the failing-requirement set $Q\!\setminus\!Q^{\mathrm{pass}}$,
% (ii) localized natural-language descriptions of what went wrong
% (e.g.\ ``the leftmost figure has three arms''), and
% (iii) concrete edit suggestions phrased in workflow terms
% (``apply regional prompting to isolate the throwing arm'').
% %
% Conditioned on this feedback, the agent loads any newly relevant skills via
% the trigger router, edits the graph into $G_{t+1}$, and resubmits it to the
% runtime, which renders a new candidate $I_{t+1}$.
% %
% Formally, the loop iterates
% \begin{equation}
%   G_{t+1} \;=\; \mathrm{Agent}\!\big(\,p,\;G_t,\;I_t,\;
%                   \underbrace{(r_t,\,Q\!\setminus\!Q^{\mathrm{pass}},\,
%                               \mathrm{desc}_t,\,\mathrm{sug}_t)}_{\text{verifier feedback}}\,\big),
%   \label{eq:repair-loop}
% \end{equation}
% until $r_t\!\geq\!\tau_{\mathrm{stop}}$ or a maximum of $K$ iterations is
% reached, whichever comes first; the iteration with the highest reward,
% $t^{\star}=\arg\max_t r_t$, is committed as the final output for prompt $p$.
% %
% The same per-iteration artefacts are also forwarded across the prompt batch
% to the skill-evolution loop in \S\ref{sec:skill-evolution}, which uses them
% to grow $\mathcal{S}$.

\subsection{Skill Evolution}
\label{sec:skill-evolution}
The skill library serves as the long-term memory of \ours{}. 
% 
Rather than treating each prompt independently, \ours{} converts recurring successes and failures across prompts into reusable workflow procedures. 
% 
Skill evolution proceeds in four stages: clustering success and failure traces, proposing skill mutations, validating the proposed mutations, and committing accepted skills to the skill library.




%
\textbf{Success and Failure Clustering.}
%
Let $\mathcal{S}^{(m)}$ denote the skill library after evolution cycle $m$.
%
After a batch of $B$ prompts, the workflow-construction loop produces traces
\begin{equation}
    \mathcal{D}^{(m)}
    =
    \left\{
    \left(p_i, G_i, x_i, r_i, f_i, e_i, a_{i,1:T_i}\right)
    \right\}_{i=1}^{B},
\end{equation}
where $p_i$ is the prompt, $G_i$ is the final workflow, $x_i$ is the generated
image, $r_i$ is the verifier reward, $f_i$ is verifier feedback, $e_i$ is a
runtime error if one occurs, and $a_{i,1:T_i}$ is the sequence of workflow
actions.
%
As shown in the bottom part of Figure~\ref{fig:overview}, these success and
failure traces are sent to the skill evolution module.

We divide traces into success and failure groups using the verifier reward.
%
A trace is treated as successful if $r_i \ge 0.9$ and as a failure otherwise.
%
We then cluster the success and failure traces separately according to their
verifier feedback, runtime errors, workflow actions, and prompt properties.
%
Failure clusters capture recurring failure modes, such as missing objects,
incorrect counting, weak spatial binding.
%
Success clusters capture reusable workflow strategies, such as when to add a LoRA, when to use regional attention, how to adjust guidance, or how to structure prompts.

\textbf{Skill Mutation.}
%
For each cluster $C_\ell$, we use the agent as a skill evolver to propose a
mutation to the current skill library.
%
The mutation type is selected from
\begin{equation}
    \mu_\ell \in
    \{\texttt{create}, \texttt{revise}, \texttt{reinforce},
      \texttt{merge}, \texttt{delete}\}.
\end{equation}
%
A \texttt{create} mutation adds a new procedure for a pattern not covered by
existing skills.
%
A \texttt{revise} mutation updates the content of an existing skill.
%
A \texttt{reinforce} mutation strengthens useful triggers or emphasis terms.
%
A \texttt{merge} mutation combines redundant skills, and a \texttt{delete}
mutation removes skills that are no longer useful.
%
Applying the proposed mutation to the current library gives a candidate skill
library
\begin{equation}
    \widetilde{\mathcal{S}}_{\ell}^{(m+1)}
    =
    \mu_\ell\!\left(\mathcal{S}^{(m)}\right).
\end{equation}

\textbf{Mutation Validation.}
%
Each candidate mutation is validated before it is committed to the skill
library.
%
For cluster $C_\ell$, we ask the agent to synthesize three held-out prompts
conditioned on the cluster identifier, the candidate skill name, and up to five
example prompts from the cluster.
%
These prompts are intended to test whether the proposed mutation generalizes
beyond the examples that produced it.
%
% If held-out prompt generation fails, we instead use three prompts from
% $C_\ell$, making the validation in-distribution.

Let $\mathcal{H}_\ell$ denote the validation prompt set for cluster $C_\ell$.
%
We compare the average verifier reward obtained with the current skill library
$\mathcal{S}^{(m)}$ against the reward obtained with the candidate library
$\widetilde{\mathcal{S}}_{\ell}^{(m+1)}$:
\begin{equation}
    \Delta_\ell
    =
    \frac{1}{|\mathcal{H}_\ell|}
    \sum_{p \in \mathcal{H}_\ell}
    \left[
    r\!\left(p;\widetilde{\mathcal{S}}_{\ell}^{(m+1)}\right)
    -
    r\!\left(p;\mathcal{S}^{(m)}\right)
    \right].
\end{equation}
%
The mutation is accepted only if it does not degrade validation performance $\Delta_\ell \ge 0.$
% \begin{equation}
    % \Delta_\ell \ge 0.
% \end{equation}
%
Rejected mutations are rolled back, while accepted mutations are committed as
new skill versions.
%
% Through this validation step, the skill library accumulates reusable procedures that improve later workflow-construction runs rather than only fitting past examples.





% \subsection{Skill-Augmented Workflow MDP}
% \label{sec:method:mdp}

% We formalize workflow synthesis for each prompt as a skill-augmented MDP,
% \begin{equation}
%   \mathcal{M} \;=\; (\Sset,\,\Aset,\,T,\,R,\,\gamma,\,\skillset).
% \end{equation}
% A state is $s=(G,p,k,h)$, where $G$ is the current workflow graph, $p$ is the
% prompt, $k$ is the current construction stage, and $h$ is the interaction
% history.
% The action space contains primitive graph operations and higher-level
% workflow macros:
% \begin{equation}
%   \Aset \;=\; \Aset_{\mathrm{add}} \cup \Aset_{\mathrm{connect}}
%               \cup \Aset_{\mathrm{param}} \cup \Aset_{\mathrm{delete}}
%               \cup \Aset_{\mathrm{meta}}.
% \end{equation}
% These actions include \texttt{add\_node}, \texttt{connect\_nodes},
% \texttt{set\_param}, \texttt{delete\_node}, \texttt{validate\_workflow},
% \texttt{finalize\_workflow}, and skill-aware macros such as
% \texttt{add\_lora\_loader}, \texttt{add\_regional\_attention},
% \texttt{add\_hires\_fix}, and \texttt{read\_skill}.
% Graph edits are deterministic, $G'=\mathrm{apply}(a,G)$.
% Rendering and verification are evaluated after each submitted workflow.

% The reward balances prompt fidelity, image detail, workflow complexity, and
% feasibility:
% \begin{equation}
%   R(s,a,s') \;=\; R_{\mathrm{qual}}(s')
%                   \;+\; R_{\mathrm{cplx}}(s')
%                   \;+\; R_{\mathrm{feas}}(s').
% \end{equation}
% The three terms are defined as
% \begin{align}
%   R_{\mathrm{qual}} &= w_{\mathrm{req}}\!\cdot\!\frac{1}{|Q|}\!\sum_{i=1}^{|Q|}\!
%                        \1\bigl[\mathrm{pass}(q_i)\bigr]
%                        \;+\; w_{\mathrm{det}}\!\cdot\!\tilde s_{\mathrm{det}}, \\
%   R_{\mathrm{cplx}} &= -\lambda\!\cdot\!\frac{\max\bigl(0,\,|V'|-N_0\bigr)}{N_0}, \\
%   R_{\mathrm{feas}} &= \begin{cases}
%     0       & G'\ \text{passes ComfyUI validation,}\\
%     -\infty & \text{otherwise.}
%   \end{cases}
% \end{align}
% Here $N_0$ is the node count of the base workflow and $\lambda=0.02$ penalizes
% unnecessary graph growth.
% Each prompt is a fresh episode, so we set $\gamma=0$.
% During an episode, the harness keeps the best-so-far tuple
% $(G^\star,x^\star,R^\star)$ and returns $x^\star$ at termination.

% A skill $\sigma\in\skillset$ acts as an option-like macro-action,
% \begin{equation}
%   \sigma=(I_\sigma,\pi_\sigma,\beta_\sigma,d_\sigma),
% \end{equation}
% where $I_\sigma$ is the initiation set, $\pi_\sigma$ is a natural-language
% workflow policy, $\beta_\sigma$ is an implicit termination condition, and
% $d_\sigma$ is the retrieval description.



% \subsection{Generate, Verify, and Repair Loop}
% \label{sec:method:agent}

% Algorithm~\ref{alg:harness} gives the main harness loop.
% At iteration $t$, the agent receives the prompt, the current workflow, the
% latest verifier feedback, and a compact memory of previous attempts.
% It first declares its intended improvement through
% \texttt{report\_evolution\_strategy}, then applies graph-editing tools until
% calling \texttt{finalize\_workflow}.
% If ComfyUI rejects the graph, the harness re-invokes the agent with the exact
% error message for up to $r_{\max}$ repair rounds.
% If the workflow renders successfully, the verifier scores the image and returns
% structured feedback for the next iteration.

% Two guards stabilize the loop.
% First, when \texttt{evolve\_from\_best} is enabled, the next iteration starts
% from $G^\star$ rather than the original base workflow.
% This preserves useful graph changes and allows incremental improvement.
% Second, if a candidate graph introduces more validation errors than the current
% best valid graph, the harness rolls back to $G^\star$ before continuing.

% \begin{algorithm}[t]
% \caption{\ours{} harness loop for a single prompt $p$.}
% \label{alg:harness}
% \begin{algorithmic}[1]
%   \Require base workflow $G_0$, threshold $\tau$, max iterations $T$,
%             max repairs $r_{\max}$, max non-productive attempts $\kappa_{\max}$
%   \State $G^\star \gets G_0$;\ \ $R^\star \gets -\infty$;\ \ $\mathcal{M}\gets\emptyset$
%   \State $t\gets 0$;\ \ $\kappa\gets 0$
%   \While{$t < T$ \textbf{and} $\kappa \le \kappa_{\max}$}
%     \State $G \gets \textsc{Copy}(G^\star)$
%     \State $G \gets \pi_\theta(G,p,\mathrm{feedback}_{t-1},\mathcal{M})$
%     \For{$j = 0,\dots,r_{\max}$}
%       \State $\mathrm{out}\gets\textsc{ComfyUI.submit}(G)$
%       \If{$\mathrm{out}$ is image}
%         \State \textbf{break}
%       \ElsIf{$j < r_{\max}$}
%         \State $G \gets \pi_\theta(G,p,\mathrm{error}(\mathrm{out}))$
%       \EndIf
%     \EndFor
%     \If{$\mathrm{out}$ is not image}
%       \State $\kappa\gets\kappa+1$;\ \ \textbf{continue}
%     \EndIf
%     \State $r_t,\,\mathrm{feedback}_t \gets V_\phi(\mathrm{out},p)$
%     \If{$r_t > R^\star$}
%       \State $G^\star,\,R^\star \gets G,\,r_t$
%     \EndIf
%     \State $\mathcal{M}\gets\mathcal{M}\cup\{(G,r_t,\mathrm{feedback}_t)\}$;\ \ $t\gets t+1$
%     \If{$r_t \ge \tau$}
%       \State \textbf{break}
%     \EndIf
%   \EndWhile
%   \State \Return $\mathrm{render}(G^\star;p)$
% \end{algorithmic}
% \end{algorithm}

% \subsection{Region-Level Verifier Feedback}
% \label{sec:method:verifier}

% The verifier is designed to produce actionable workflow feedback rather than
% only a scalar score.
% For each generated image, it reports which prompt requirements pass or fail,
% assigns a detail score, and identifies localized issues.
% Each region-level issue specifies the affected area, error type, severity, and
% candidate interventions.
% Interventions may include adding a regional prompt, inserting a LoRA, adding a
% hires-fix pass, refining the negative prompt, changing sampler settings, or
% adjusting guidance strength.

% This feedback distinguishes \ours{} from prompt-only refinement.
% The verifier does not merely state that an image is poor.
% It points the agent toward concrete workflow operations that can repair the
% observed failure.

% \subsection{Stage-Gated Action Space}
% \label{sec:method:stages}

% The full workflow-editing tool set is large, but only a subset is relevant at
% each construction phase.
% We therefore use a lightweight stage router that controls which tool schemas
% are visible to the agent:
% \begin{equation}
%   \Aset(k) \;\subset\; \Aset, \qquad
%   \Aset \;=\; \bigsqcup_{k=1}^{K}\Aset(k)\;\cup\;\Aset_{\mathrm{meta}}.
% \end{equation}
% We use five stages:
% \texttt{planning}, \texttt{construction}, \texttt{conditioning},
% \texttt{enhancement}, and \texttt{finalization}.
% The agent can move between stages with the \texttt{transition\_stage} meta-tool.
% This stage structure acts as a soft workflow grammar.
% It keeps irrelevant tools out of context while still allowing the agent to
% inspect and revise the graph throughout construction.

% \begin{table}[t]
% \centering
% \small
% \caption{Stage-gated tool exposure.
% Inspection and stage-transition tools remain available throughout.
% \texttt{read\_skill} is available before finalization and omitted from the
% final validation stage.}
% \label{tab:stages}
% \begin{tabular}{ll}
% \toprule
% \textbf{Stage} & \textbf{Visible tools} \\
% \midrule
% planning      & \texttt{query\_available\_models}, \texttt{report\_evolution\_strategy} \\
% construction  & \texttt{add\_node}, \texttt{connect\_nodes}, \texttt{delete\_node}, \texttt{set\_param} \\
% conditioning  & \texttt{set\_prompt}, \texttt{add\_regional\_attention}, \texttt{set\_param} \\
% enhancement   & \texttt{add\_lora\_loader}, \texttt{add\_hires\_fix}, \texttt{add\_inpaint\_pass}, base graph edits \\
% finalization  & \texttt{validate\_workflow}, \texttt{finalize\_workflow}, \texttt{set\_param}, \texttt{delete\_node} \\
% \bottomrule
% \end{tabular}
% \end{table}

% \subsection{Skill Library and Self-Evolution}
% \label{sec:method:skills}

% The skill library $\skillset$ is a directory of \texttt{SKILL.md} files.
% Built-in skills are curated and read-only.
% Evolved skills are stored separately for each
% \texttt{(model, benchmark, agent)} setting, so model-specific and
% benchmark-specific lessons do not leak across experimental conditions.

% After a benchmark rollout, the skill evolver receives records
% \[
%   D \;=\; \bigl\{\bigl(p_i,\,r_i,\,\mathrm{passed}_i,\,\mathrm{failed}_i,\,
%                   \mathrm{feedback}_i,\,\mathrm{tools}_i,\,G_i\bigr)\bigr\}.
% \]
% It clusters low-scoring examples into reusable failure patterns and
% high-scoring examples into reusable strategies.
% For each cluster, it proposes one typed mutation to the skill library:
% \texttt{create}, \texttt{update}, \texttt{merge}, \texttt{delete}, or
% \texttt{reinforce}.
% Each mutation must include trigger phrases, a compact description, and concrete
% node-level workflow instructions.

% Before a mutation is committed, the updated skill library is evaluated on
% held-out prompts generated from the same cluster.
% A mutation is accepted only if it improves the held-out score by a margin and
% does not cause any held-out prompt to regress beyond a tolerance.
% The validation score uses the same graph-complexity prior as the main loop:
% \begin{equation}
%   \overline{\mathbf{q}}^{\,\star}
%   \;=\; \overline{\mathbf{q}}
%         \;-\; \lambda\!\cdot\!\frac{\max(0,\,\bar n-N_0)}{N_0},
% \end{equation}
% where $\bar n$ is the mean node count after applying the mutation.
% Accepted mutations update the running skill library before later mutations are
% tested, so later skills are evaluated against the current library rather than a
% stale baseline.

% \subsection{Cross-Prompt Experience and Curriculum}
% \label{sec:method:memory}

% Within a prompt, \ours{} stores attempted workflows, scores, passed and failed
% requirements, verifier feedback, and the agent's self-summary in an episodic
% memory block.
% This memory is shown before each edit and helps the agent avoid repeating
% failed changes.

% Across prompts, \ours{} records
% $(p,r,G,\mathrm{passed},\mathrm{failed})$ in a SQLite experience database.
% Entries are indexed by topology hash and lightweight prompt similarity.
% For a new prompt, the system may warm-start from the highest-scoring topology
% retrieved from a similar past prompt if its relevance exceeds $0.6$.

% For benchmark runs, \ours{} also caches the unmodified base-workflow output
% using the key
% $\mathrm{sha256}(G_{\mathrm{base}},p,\mathrm{model})$.
% If this cached baseline already exceeds the target threshold $\tau$, the run
% stops.
% Otherwise, the evolutionary loop must improve over that baseline.
% For studying skill emergence, we train skills over increasingly difficult
% prompt curricula and report transfer as the fraction of accepted skills from
% one difficulty level that fire and improve scores at the next level.

\input{figures/main_results_table.tex}

\section{Experiments}
\label{sec:results}


% In this section, we run \ours{} on four image generation benchmarks with comparative baselines. We then perform ablation study and qualitative evaluation on the results to show the iterative refinement process of \ours{}.
In this section, we evaluate \ours{} on four text-to-image benchmark splits against competitive baselines. We further present ablation studies and qualitative analyses that illustrate how \ours{} improves through iterative workflow refinement.


% \textbf{Benchmarks.} We evaluate on four complementary text-to-image benchmarks selected to cover four capabilities: compositional reasoning, dense prompt following, multi-axis fidelity, and world knowledge.
% %
% \textbf{GenEval~2}~\cite{kamath2025geneval} is a compositional benchmark of 800 English prompts spanning 40 objects, 18 attributes, and 9 spatial or numerical relations. It is scored with an atom-level VQA judge (Soft-TIFA), which was introduced to reduce the saturation issues observed in the original GenEval.
% %
% \textbf{DPG-Bench}~\cite{hu2024ella} contains 1{,}065 dense English prompts that combine multiple objects, attributes, and relations within a single sentence, making it a strong test of faithful rendering for long, structured descriptions.
% %
% \textbf{OneIG-Bench}~\cite{chang2025oneig} provides a fine-grained multi-axis evaluation covering subject--element alignment, text rendering, reasoning content, stylization, and diversity. We use both its 1{,}120-prompt English split (\textbf{OneIG-EN}) and its 1{,}320-prompt Chinese split (\textbf{OneIG-ZH}) to evaluate cross-lingual generalization.
% %
% Taken together, these five benchmarks comprise approximately 4{,}300 prompts and cover the four dimensions along which agentic workflow evolution is most likely to differ from prompt-only refinement.


\textbf{Benchmarks.}
We evaluate on four text-to-image benchmark splits covering compositional reasoning, dense prompt following, fine-grained fidelity, and cross-lingual generalization.
%
\textbf{GenEval~2}~\cite{kamath2025geneval} includes 800 English prompts over objects, attributes, and spatial or numerical relations, scored with the atom-level Soft-TIFA VQA judge to avoid saturation in the original GenEval.
%
\textbf{DPG-Bench}~\cite{hu2024ella} contains 1{,}065 dense English prompts with multiple objects, attributes, and relations in each sentence.
%
\textbf{OneIG-Bench}~\cite{chang2025oneig} evaluates subject--element alignment, text rendering, reasoning content, stylization, and diversity. We use its English split (\textbf{OneIG-EN}, 1{,}120 prompts) and Chinese split (\textbf{OneIG-ZH}, 1{,}320 prompts).
%
Together, these benchmarks contain roughly 4{,}300 prompts and test the dimensions where workflow evolution should differ most from prompt-only refinement.

% \textbf{Agents and ComfyUI models used.}
% %
% We use three foundation models as workflow control agents: one proprietary model, Claude Sonnet 4.5~\cite{anthropic2025claude}, and two open-source models, Qwen-3.6-35B-A3B~\cite{yang2025qwen3} and Gemma-4-E4B-it~\cite{gemma4_2026}.
% %
% All three are natively multimodal models that accept both text and images as input. We use them to instantiate the workflow agent, verifier agent, and skill-evolution agent in our system.
% %
% For image generation, we evaluate two backbone models: z-image-turbo~\cite{cai2025z}, a 6B-parameter text-to-image model, and LongCat-Image~\cite{team2025longcat}, a 6B-parameter open-source bilingual (Chinese--English) foundation model for image generation and editing.
% %
% The agents operate over the ComfyUI workflow graph and instruct the underlying ComfyUI pipeline to generate images with these image generation models.

\textbf{Agents and ComfyUI models used.}
We use three foundation models as workflow-control agents: Claude Sonnet
4.5~\cite{anthropic2025claude}, Qwen-3.6-35B-A3B~\cite{yang2025qwen3}, and Gemma-4-E4B-it~\cite{gemma4_2026}. 
%
All are natively multimodal and are used to instantiate the workflow, verifier, and skill-evolution agents. 
%
For image generation, we evaluate two ComfyUI backbones: z-image-turbo~\cite{cai2025z}, a 6B text-to-image model, and LongCat-Image~\cite{team2025longcat}, a 6B bilingual Chinese--English model for image generation and editing. 
%
The agents edit the ComfyUI workflow graph, while the selected backbone renders the final image.


\textbf{Workflow and tool setup.}
%
To closely simulate how an external agent would control a real ComfyUI deployment, we instantiate a fresh ComfyUI server endpoint for each experimental condition.
%
Each endpoint runs an unmodified ComfyUI server, while our agent is deployed as an external plug-in that submits jobs and retrieves execution logs through the standard interface.
%
This design allows our framework to interact with ComfyUI without modifying the application itself, making the setup easy to maintain and naturally compatible with any future ComfyUI updates.
%

We provide a set of workflow-editing tools for controlling ComfyUI workflows,
together with four predefined visual-quality skills by~\citet{he2026gems}.
%
During execution, the agent does more than prompt rewriting: it can edit the workflow graph, tune node hyperparameters, and, when supported by the image model, attach and configure LoRAs.
%
The full list of predefined tools, predefined skills, and model-specific LoRA settings is provided in Appendix~\ref{app:tools-skills}.


\textbf{Image Generation Evaluation Metrics.}
We follow the headline metric defined by each benchmark.
%
For GenEval2, we report the Soft-TIFA geometric mean~\cite{hu2023tifa} (gm), computed over the per-prompt set of VQA questions, including yes/no and counting questions~\cite{lin2024evaluating}.
%
For DPG-Bench, we report the Soft-TIFA arithmetic mean (am), computed over each prompt’s corresponding set of evaluation questions.
%
For OneIG-EN and OneIG-ZH, we use VQAScore, where each image is evaluated with a single query of the form: \textit{Does this image show \textit{<prompt>}? Answer Yes or No.}
%
All of these metrics rely on a VLM-as-a-judge.
%
In our experiments, we use Qwen3-VL-8B-Instruct~\cite{bai2025qwen3} as the primary judge model to answer the benchmark evaluation queries.


\subsection{Main Results}
%
% We evaluate two experimental groups.
% %
% \ours{} starts with an agent that controls the ComfyUI workflow and iteratively refines it to generate better images using verifier feedback.
% %
% During workflow construction, the agent has access to the full set of tools and skills. It can also evolve new skills from ComfyUI execution errors, successful runs, and high verifier scores.
%
We compare \ours{} against two baseline groups.
%
The first baseline, \baseline{}, uses only the initial tools and skill set. It does not receive verifier feedback or perform refinement; instead, it executes the workflow once and directly returns the generated image.
%
The second baseline has access to the full tool and skill set and uses a verifier-guided refinement loop to improve the generated image, but it does not perform skill evolution.
%
All experiments and evaluations are done on RTX PRO 6000 Blackwell GPU with 96 GB memory. 
%
We report the results in Table~\ref{tab:results1}.
%
Overall, \ours{} outperforms both \baseline{} and \comfygems{} across all four benchmarks.
%
These results suggest two main takeaways.
%
First, adding a VLM verifier and refinement loop helps agents construct better workflows and generate higher-quality images.
%
Second, skill evolution further improves performance by enabling agents to summarize successes and failures, learn from past errors, and update their skill set for future workflow construction.
%


% % \textbf{Error Rates and success failures...}



% \begin{table}[!htbp]
%     \centering
%     \small
%     \begin{tabular}{lrrrrr}
%       \toprule
%       Benchmark & Evolved Skills & Total Reads & Base Reads & Evolved Reads & \% Evolved Reads \\
%       \midrule
%       dpg-bench  &  62 &  9,251 &  2,078 &  6,478 & 70.0\% \\
%       geneval2   &  79 & 20,282 &  5,377 & 11,391 & 56.2\% \\
%       oneig-en   &  60 &  5,355 &  3,334 &    872 & 16.3\% \\
%       oneig-zh   & 118 &  3,266 &  2,747 &    244 &  7.5\% \\
%       \midrule
%       \textbf{TOTAL} & \textbf{318} & \textbf{38,154} & \textbf{13,536} & \textbf{18,985} & \textbf{49.8\%} \\
%       \bottomrule
%     \end{tabular}
%     \caption{Total number and percentage of evolved skill usage per benchmark on Claude-Sonnet-4.5 for Longcat-Image and Z-Image-turbo. The percentage of evolved skills are used heavily read and used by the agent to construct the workflow to create images. \wxy{can we use a figure here?}}
%     \label{tab:evolved}
% \end{table}

\input{figures/fig_table.tex}

\textbf{Evolved skills are heavily used by agents.}
%
We analyze the skills evolved by Claude-Sonnet-4.5 across four benchmarks and two image-generation models.
%
As shown in Figure~\ref{fig:evolved_reads}, evolved skills account for an average of $\sim\!50\%$ of total skill reads across benchmarks (specifically $70.0\%$ on DPG-Bench and $56.2\%$ on GenEval2, dropping to $16.3\%$ on OneIG-EN and $7.5\%$ on OneIG-ZH), indicating that agents rely heavily on them when constructing image-generation workflows for dense and compositional prompts.
%
Across the eight experimental settings, Claude-Sonnet-4.5 produced $318$ unique skills, totaling $4{,}768$ skill versions.
%
These skills reflect the distinct requirements of each benchmark.
%
GenEval2 primarily induces object-counting and attribute-binding skills; DPG-Bench emphasizes spatial relations, poses, and anatomy; OneIG-EN favors anime-style prompting and character-count control; and OneIG-ZH further introduces Chinese-specific anime conventions and resolution-tag skills.\footnote{The top ten evolved skills are listed in Appendix~\ref{app:evolved_skills}.}
%
The evolved skills provide reusable, task-specific patterns that help agents start from stronger knowledge and generate higher-quality images.

% \begin{table}[!htbp]
%     \centering
%     \small
%     \setlength{\tabcolsep}{6pt}
%     \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{l r r r r r r}
%     \toprule
%     \textbf{Workflow Event} &
%     \textbf{DPG-Bench} & \textbf{GenEval2} & \textbf{OneIG-EN} & \textbf{OneIG-ZH} &
%     \textbf{Total} & \textbf{\%} \\
%     \midrule
%     Prompt-text changes              & 2{,}862 & 4{,}139 & 3{,}277 & 3{,}714 & 13{,}992 & 39.3\% \\
%     Sampler / guidance hyper-params  & 2{,}776 & 2{,}415 & 3{,}408 & 4{,}161 & 12{,}760 & 35.8\% \\
%     Regional / mask graph topology   &    214  & 2{,}958 &    484  &    400  &  4{,}056 & 11.4\% \\
%     Model / weight changes (LoRA, ckpt) & 570 &    518  &    721  &    806  &  2{,}615 &  7.3\% \\
%     Multi-pass / upscale topology    &    195  &    258  &    328  &    358  &  1{,}139 &  3.2\% \\
%     Other (class swaps, removes, misc)& 114    &    599  &    170  &    167  &  1{,}050 &  2.9\% \\
%     \midrule
%     \textbf{Total events}            & \textbf{6{,}731} & \textbf{10{,}887} & \textbf{8{,}388} &
%                                        \textbf{9{,}606} & \textbf{35{,}612} & \textbf{100.0\%} \\
%     \bottomrule
%     \end{tabular}
%     }% end resizebox
%     \caption{Action-event breakdown for workflow construction in \ours{}. Each \emph{event} denotes a node-level workflow change: adding a node, removing a node, or editing a node's \texttt{inputs} field. For each benchmark, counts are aggregated over the two image-generation models, \textsc{LongCat} and \textsc{Z-Image-Turbo}.}
%     \label{tab:modification-breakdown}
% \end{table}


% \textbf{components of different workflows used to show that it is not just prompt engineering.}

\textbf{Agents perform more complex actions than simple prompt rewriting.}
%
We track the actions taken by the Claude agent when constructing workflows in \ours{}, as shown in Figure~\ref{fig:modification_breakdown}.
%
Across $35{,}612$ workflow events, prompt-text edits are the most frequent single category but account for only $39.3\%$ of all edits.
%
The remaining $60.7\%$ modify other parts of the workflow, including sampler and guidance hyperparameters ($35.8\%$), regional or mask-based graph topology ($11.4\%$, with a striking $27\%$ on GenEval2), LoRA / checkpoint selection ($7.3\%$), and multi-pass upscaling ($3.2\%$).
%
This shows that \ours{} improves image generation through broader workflow optimization rather than relying only on prompt refinement.


% \textbf{Better agent make tool use and more skills and verifier better. If agent not good enough, the baseline with few skills is better because involve in less planning. However, with skill evolvement, the agent is being able to learn from errors and success to avoid over-complicated planning and directly use skills. Show some example skills.}


% \textbf{\ours{} generates }

\input{figures/comfyclaw_cherrypick_figure.tex}

% \textbf{How often are Loras used?}

\FloatBarrier

\subsection{Qualitative Analysis}
We further conduct a qualitative analysis of the generated images, since quantitative metrics alone may not fully capture visual quality in image generation tasks.
%
Our goal is to compare how different harness designs affect the agent's ability to control the workflow and produce high-quality images.
%
We hire two annotators to rate image quality on a 1--5 Likert scale, where higher scores indicate better visual quality and stronger text-image alignment.
%
For each benchmark and each agent, we randomly sample 50 finalized images.
%
Annotators are shown the input prompt together with the generated images from different experimental groups, and are asked to assign a Likert rating to each image.\footnote{Annotation cost and instruction details are in Appendix~\ref{app:user_study}}
%
In total, 2{,}400 images are annotated.
%
We show the results in Table~\ref{tab:qualitative_evals}.
%
Overall, images generated using \ours{} align more with input prompts, while brings more visual realism and asthetics.


\begin{table}[!htbp]
  \centering
  \small
  \resizebox{0.8\columnwidth}{!}{%
  \begin{tabular}{llccccc}
    \toprule
    Image Model & Method & GenEval2  & DPG-Bench  & OneIG-EN  & OneIG-ZH  & Avg \\
    \midrule
    \multirow{3}{*}{\texttt{longcat}} & \baseline{} & 3.63 & 3.81 & 3.50 & 3.64 & 3.65 \\
    & \comfygems{} & 4.01 & 4.33 & 4.10 & 3.94 & 4.10 \\
    & \ours{} & \textbf{4.02} & \textbf{4.74} & \textbf{4.55} & \textbf{4.66} & \textbf{4.49} \\
    \midrule
    \multirow{3}{*}{\texttt{z-image-turbo}} & \baseline{} & 3.58 & 4.54 & 4.42 & 4.48 & 4.26 \\
     & \comfygems{} & 3.98 & \textbf{4.63} & 4.34 & 4.49 & 4.36 \\
     & \ours{} & \textbf{4.36} & 4.60 & \textbf{4.59} & \textbf{4.55} & \textbf{4.53} \\
    \bottomrule
  \end{tabular}
  }% end resizebox
  \caption{\textbf{Qualitative evaluation of Claude as an agent to control the ComfyUI workflow.} Overall \ours{} has higher average human visual annotation scores than \comfygems{} and \baseline{}.}
  \label{tab:qualitative_evals}
  \vspace{-10pt}
\end{table}






\textbf{Closed-loop workflow refinement repairs failures that
prompt-only rewriting often cannot.}
%
Figure~\ref{fig:comfyclaw-refinement} shows \ours{}'s refinement loop for editing the workflow.
%
\textit{First}, the edits are structural rather than purely textual prompt revision.
%
In Figure~\ref{fig:comfyclaw-refinement}(a), the agent stacks two
Z-Image LoRAs and adds a regional-attention block before the unusual attribute
\emph{purple} is correctly bound to all four lions.
%
In Figure~\ref{fig:comfyclaw-refinement}(b), the agent adjusts the regional
split until the spatial relation \emph{left of}, the material \emph{glass},
and the count \emph{three} are all satisfied.
%

\textit{Second}, refinement is not always monotonic.
%
Some intermediate attempts are worse than the baseline, such as when the pigs
disappear or the clock is lost, but the best-so-far buffer preserves the best
valid candidate while still allowing the agent to learn from failed attempts
and recover in later iterations.
%

\textit{Third}, the loop is verifier-driven.
%
Each refinement instruction directly responds to the preceding critique, such
as correcting the lion color or removing an ineffective LoRA after objects
disappear.
%
Thus, the agent is not retrying blindly; it spends additional graph edits and
re-renders on the specific failures localized by the verifier.
%
These extra operations improve compositional errors, including
attribute binding, object count, and spatial relations, Lora weight stacking, hyperparameter adjustments that are difficult for
single-pass prompt-only generation to fix reliably.

\input{figures/comfyclaw_refinement_figure}



\FloatBarrier

% \subsection{Discussion}

\section{Conclusion}
\label{sec:conclusion}
Agentic workflow control is a promising direction for helping users, especially beginners, operate complex tools and automate multi-step workflows.
%
In image generation, workflow-based systems provide more controllability than prompt-only interfaces by exposing components such as model selection,
conditioning, sampling, refinement, and LoRA adapters.
%
We propose \ours{}, a self-evolving workflow-control framework that converts past successes and failures into reusable skills, enabling agents to improve how they construct and refine image-generation workflows over time.
%
Our experiments show that this self-evolving skill mechanism produces higher quality and more realistic images than agent workflow control without skill evolution, and is preferred more often by human annotators.
%
These results suggest that effective visual generation agents should not only execute workflows, but also learn and evolve reusable workflow procedures from their own experience.



\section{Limitations and Future Work}
\label{sec:limitation}

Our current study focuses only on image-generation workflows.
%
However, ComfyUI also supports video-generation workflows, which require more
complex node control, scene planning, frame consistency, and temporal
conditioning.
%
Video generation also requires substantially more compute and longer execution
time, making agent control more difficult because long-running workflows can
increase latency, timeout failures, and response errors.
%
We therefore leave video workflow control as an important direction for future
work.
%
Future systems will need stronger workflow-control strategies, better skill
management, and more efficient skill retrieval, since video workflows are
typically longer and more complex than image workflows.
%
Managing the agent context window will also become more challenging, making
compact and accurate skill retrieval especially important.

\section{Predefined Tools, Skills, and LoRA Settings}
\label{app:tools-skills}

\paragraph{Workflow tools.}
We expose 17 basic tools for controlling ComfyUI workflows.
%
These tools allow the agent to inspect the current workflow, add and remove
nodes, connect nodes, edit node inputs, set prompts, configure model-specific
parameters, validate the workflow, and submit the final graph for rendering.
%
Examples include \textsc{add\_node}, \textsc{set\_prompt}, and
\textsc{set\_lora}.
%
Together, these tools allow the agent to construct and repair workflows at the
graph level rather than only rewriting the text prompt.

\paragraph{Predefined skills.}
In addition to evolved skills, we provide four predefined skills inspired
by~\citet{he2026gems}: \textsc{photorealistic}, \textsc{creative},
\textsc{high-quality}, and \textsc{prompt-artist}.
%
These skills provide general image-generation guidance, such as improving
photorealism, increasing visual creativity, enhancing overall quality, and
rewriting prompts for stronger visual composition.
%
They serve as the initial reusable skill library before benchmark-specific
skills are evolved.

\paragraph{Model-specific LoRA settings.}
For \textsc{Z-Image-Turbo}, we include two LoRAs.
%
The first is a realistic snapshot LoRA~\cite{zimage2025,realisticsnapshot2026},
which encourages more photorealistic and real-life imagery.
%
The second is an enhancer LoRA~\cite{enhancer2026}, which improves generation
quality across a range of visual styles.
%
\textsc{LongCat-Image} does not currently support LoRAs in our setup, so
LoRA-based tools are disabled for that model.

\begin{table}[!htbp]
\centering
\small
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}p{0.21\linewidth}p{0.38\linewidth}p{0.35\linewidth}@{}}
\toprule
\textbf{Group} & \textbf{Tool} & \textbf{Purpose} \\
\midrule
\multirow{3}{*}{\textit{Inspection}}
  & \texttt{inspect\_workflow}        & Summarise nodes, IDs, classes, inputs of the current graph. \\
  & \texttt{query\_available\_\newline{}models} & List installed checkpoints / LoRAs / UNETs / VAEs / upscalers. \\
  & \texttt{explore\_nodes}           & Query \texttt{/object\_info} and classify nodes by pipeline stage. \\
\midrule
\multirow{4}{*}{\textit{Graph edits}}
  & \texttt{add\_node}      & Append a node; return its new ID. \\
  & \texttt{connect\_nodes} & Wire \emph{src}.slot $\to$ \emph{dst}.input. \\
  & \texttt{delete\_node}   & Remove a node and its incident links. \\
  & \texttt{set\_param}     & Set a scalar input on a specific node. \\
\midrule
\multirow{5}{*}{\textit{Composite macros}}
  & \texttt{set\_prompt}              & Set positive/negative text on every encoder feeding a sampler. \\
  & \texttt{add\_lora\_loader}        & Insert a LoRA between model source and downstream consumers. \\
  & \texttt{add\_regional\_\newline{}attention} & Split conditioning into foreground/background regional prompts. \\
  & \texttt{add\_hires\_fix}          & Add latent upscale + second \texttt{KSampler} + \texttt{VAEDecode}. \\
  & \texttt{add\_inpaint\_pass}       & Add a targeted inpaint pass for a specific region. \\
\midrule
\textit{Skills}
  & \texttt{read\_skill}              & Load a \texttt{SKILL.md} body by name (progressive disclosure). \\
\midrule
\multirow{4}{*}{\textit{Control / meta}}
  & \texttt{report\_evolution\_\newline{}strategy} & Declare the iteration plan and top issue before edits. \\
  & \texttt{validate\_workflow}          & Check the graph for dangling refs, wrong slots, missing outputs. \\
  & \texttt{finalize\_workflow}          & Signal completion (auto-validates; blocks if errors remain). \\
  & \texttt{transition\_stage}           & Advance through planning $\to \cdots \to$ finalization. \\
\bottomrule
\end{tabular}%
\caption{The 17 predefined tools the agent uses to construct and repair
ComfyUI workflows, grouped by function.  Composite macros bundle a
sequence of base graph edits with the correct rewiring and slot binding.
% Stage gating (\S\ref{sec:method:stages}) further restricts which subset is visible at each pipeline stage.
}
\label{tab:tools}
\end{table}

\begin{table}[!htbp]
\centering
\scriptsize
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{0.24\linewidth}p{0.34\linewidth}p{0.33\linewidth}@{}}
\toprule
\textbf{Skill} & \textbf{When to consult (trigger phrases)} & \textbf{Effect on the workflow} \\
\midrule
\texttt{photorealistic}
  & ``photo'', ``photograph'', ``realistic'', ``DSLR'', ``cinematic'',
    ``RAW photo'', ``shot on $\langle$camera$\rangle$''; or ``make it look real''.
  & Rewrites positive/negative prompts toward camera realism; tunes
    KSampler steps, CFG, and sampler/scheduler for natural lighting and
    DSLR-like fidelity. \\
\addlinespace
\texttt{creative}
  & ``creative'', ``artistic'', ``fantasy'', ``concept art'', ``surreal'',
    ``stylized''; clearly fictional scenes where photorealism is wrong.
  & Sets sampler parameters and prompt tags for vivid, concept-art-style
    outputs.  Pairs with \texttt{prompt-artist} for prompt enrichment. \\
\addlinespace
\texttt{high-quality}
  & ``high quality'', ``detailed'', ``sharp'', ``crisp'', ``professional'',
    ``8K''; or verifier reports of soft detail or noise.
  & Layered on top of \texttt{photorealistic}/\texttt{creative}: tunes
    prompt tokens, sampler parameters, and resolution to lift fidelity. \\
\addlinespace
\texttt{prompt-artist}
  & ``aesthetic'', ``dreamy'', ``masterpiece'', ``award-winning'',
    ``imaginative''; or sparse, flat user prompts.
  & Rewrites a flat prompt into vivid multi-dimensional artistic language;
    returns prompt text only and pairs with parameter-tuning skills. \\
\bottomrule
\end{tabular}
}
\caption{The four general-purpose skills loaded into every run before any
benchmark-specific evolution.  Each is a \texttt{SKILL.md} package with
YAML frontmatter exposing only the description at startup; the full body
is loaded on demand via \texttt{read\_skill}.}
\label{tab:skills}
\end{table}

\section{Evolved Skill Usage}
\label{app:evolved_skills}
Table~\ref{tab:top10-evolved} provides a usage-level view of the skills produced
by the Claude-Sonnet-4.5.  
%
Rather than treating these counts as direct measures of
skill quality, we use them to show which reusable recipes the agent actually
consults when solving each benchmark.  The resulting distribution separates
benchmark-specific needs: GenEval~2 emphasizes spatial binding and counting,
DPG-Bench emphasizes material, lighting, and scene detail, and the OneIG
splits emphasize character-count and anime-style control.

\begin{table}[t]
\centering
\scriptsize
\renewcommand{\arraystretch}{1.05}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}c p{0.36\linewidth} r p{0.34\linewidth} r@{}}
\toprule
\textbf{\#}
 & \multicolumn{2}{c}{\textbf{GenEval 2}}
 & \multicolumn{2}{c}{\textbf{DPG-Bench}} \\
\cmidrule(lr){2-3}\cmidrule(l){4-5}
 & \textbf{Skill} & \textbf{Reads}
 & \textbf{Skill} & \textbf{Reads} \\
\midrule
1  & \path|spatial-anchor-with-count|     & 1523 & \path|material-texture-detail|         &  980 \\
2  & \path|spatial-count-binding|         & 1316 & \path|spatial-precision|               &  696 \\
3  & \path|attribute-binding|             &  828 & \path|precise-color-attribution|       &  692 \\
4  & \path|material-modifier|             &  771 & \path|contextual-environment-building| &  591 \\
5  & \path|animal-color-override|         &  633 & \path|lighting-and-reflection-detail|  &  572 \\
6  & \path|exact-seven-count|             &  395 & \path|material-texture-encoding|       &  556 \\
7  & \path|animal-pattern-count|          &  386 & \path|layered-scene-building|          &  348 \\
8  & \path|high-total-count-coordinator|  &  370 & \path|visual-contrast-encoding|        &  297 \\
9  & \path|count-six-five-flock|          & ---  & \path|explicit-colors|                 &  271 \\
10 & \path|spatial-binding-three-objects| & ---  & \path|anatomy-pose-detail|             & ---  \\
\bottomrule
\end{tabular}

\vspace{4pt}

\begin{tabular}{@{}c p{0.36\linewidth} r p{0.34\linewidth} r@{}}
\toprule
\textbf{\#}
 & \multicolumn{2}{c}{\textbf{OneIG-EN}}
 & \multicolumn{2}{c}{\textbf{OneIG-ZH}} \\
\cmidrule(lr){2-3}\cmidrule(l){4-5}
 & \textbf{Skill} & \textbf{Reads}
 & \textbf{Skill} & \textbf{Reads} \\
\midrule
1  & \path|character-counting|                 & 166 & \path|anime-single-character-simple|      & 44  \\
2  & \path|anime-danbooru-ordering|            & 126 & \path|anime-multi-character|              & 33  \\
3  & \path|anime-character-counting|           & 124 & \path|detailed-character-design|          & 33  \\
4  & \path|anime-style-declaration|            &  95 & \path|anime-solo-simple|                  & 21  \\
5  & \path|presentation-slide-text|            &  61 & \path|anime-character-state-verification| & 19  \\
6  & \path|presentation-chart-internal-labels| &  20 & \path|chinese-group-counting|             & 18  \\
7  & \path|presentation-diagram-structure|     &  17 & \path|anime-direct-tag-format|            & 16  \\
8  & \path|rate-limit-mitigation|              &  15 & \path|resolution-quality-tags|            & 15  \\
9  & \path|anime-style-tag|                    & --- & \path|anime-square-resolution|            & --- \\
10 & \path|character-state-control|            & --- & \path|chinese-stylized-prompt|            & --- \\
\bottomrule
\end{tabular}

\caption{Top-10 evolved skills per benchmark for Claude-Sonnet-4.5.  Counts are total \texttt{read\_skill} calls aggregated over all prompts and both image backbones (Z-Image-Turbo and LongCat-Image).  We exclude two run-level aggregator skills so the table reflects topical recipes rather than bookkeeping.}
\label{tab:top10-evolved}
\end{table}
\footnotetext{We omit the run-level aggregator skills
\texttt{learned-successes} and \texttt{learned-errors}, which summarise each
cycle's success and failure clusters rather than encoding topical recipes.
Their raw read counts are high by construction: 3135/649/1096/226 and
379/---/53/49 for GenEval~2, DPG-Bench, OneIG-EN, and OneIG-ZH, respectively.}

\begin{table}[!htbp]
\centering
\small
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{0.18\linewidth}p{0.30\linewidth}rp{0.26\linewidth}p{0.15\linewidth}@{}}
\toprule
\textbf{Model} & \textbf{LoRA file} & \textbf{Size} & \textbf{Focus} & \textbf{Default strength} \\
\midrule
Z-Image-\newline{}Turbo
  & {\ttfamily Z-Image-Turbo-\newline{}Radiant-Realism-\newline{}Pro.safetensors} & $\sim$163\,MB
  & Realism + lighting polish (``enhancer'')       & 0.80 \\
  & {\ttfamily Z-Image-Turbo-\newline{}Realism-LoRA.\newline{}safetensors}         & $\sim$82\,MB
  & Lighter realism tweak (``realistic snapshot'') & 0.70 \\
\addlinespace
LongCat-Image & \multicolumn{4}{p{0.74\linewidth}@{}}{\textit{--- not supported in our setup ---}} \\
\bottomrule
\end{tabular}
}
\caption{Model-specific LoRA settings used in our experiments.
Z-Image-Turbo is an S3-DiT architecture, so all LoRAs are injected via
\texttt{LoraLoaderModelOnly} (model-only, no CLIP weights).  LongCat-Image
exposes no model tensor compatible with our LoRA tools, so they are
disabled for that backbone.  Strengths follow the recipe in the
\texttt{z-image-turbo} skill.}
\label{tab:loras}
\end{table}

\section{Qualitative Annotations}
\label{app:user_study}
For the user study, each participant was given the instruction template in Box~\ref{box:eval-instructions} and asked to annotate generated images. 
% 
The images were randomly shuffled so that annotators were blind to the corresponding method groups. 
% 
Annotators were paid $\$0.10$ per image, for a total of 2{,}400 annotations and $\$240$ in compensation. 
% 
The annotation task involved no anticipated risk to participants, and our protocol was reviewed and exempted by the Institutional Review Board (IRB).

\begin{tcolorbox}[
  colback=gray!5,
  colframe=gray!60,
  title={\textbf{Evaluation Instructions}},
  fonttitle=\sffamily\bfseries,
  boxrule=0.5pt,
  arc=2pt
]
\label{box:eval-instructions}
Rate the overall result on a \textbf{1--5 scale} that combines three criteria:

\begin{enumerate}[label=(\alph*),leftmargin=2em,itemsep=2pt]
  \item \textbf{Prompt--image alignment} --- Does the image faithfully depict
        the objects, attributes, count, relationships, and style specified in
        the prompt?
  \item \textbf{Visual aesthetic} --- Composition, lighting, colour, and
        balance.
  \item \textbf{Image quality} --- Sharpness, absence of artifacts, anatomical
        and structural correctness, no distorted text/hands/faces.
\end{enumerate}

\vspace{6pt}
\renewcommand{\arraystretch}{1.35}
\begin{tabularx}{\linewidth}{c >{\raggedright\arraybackslash}X}
  \toprule
  \textbf{Score} & \textbf{Description} \\
  \midrule
  1 & \emph{Very poor} --- badly misaligned with the prompt, or severely
      flawed image. \\
  2 & \emph{Poor} --- notable misalignment \textbf{or} notable quality
      issues. \\
  3 & \emph{Average} --- acceptable but with visible alignment \textbf{or}
      quality issues. \\
  4 & \emph{Good} --- well-aligned and visually appealing; only minor
      issues. \\
  5 & \emph{Excellent} --- faithfully depicts the prompt \textbf{and} looks
      polished. \\
  \bottomrule
\end{tabularx}

\end{tcolorbox}


\section{LLM Prompts}
\label{app:prompts}

This section lists the exact prompts used in the implementations of the agent loop
(\S\ref{sec:method:workflow-construction}) and the region-level VLM verifier
(\S\ref{subsec:vlm-verifier}).
All prompts are drawn verbatim from \texttt{comfyclaw/agent.py},
\texttt{comfyclaw/verifier.py}, and \texttt{comfyclaw/harness.py}.

% -----------------------------------------------------------------------
\subsection{Agent System Prompt (\S\ref{sec:method:workflow-construction})}
\label{app:prompts:system}

The following string (\texttt{\_SYSTEM\_PROMPT\_BASE}) is prepended to every
agent conversation as the \texttt{system} role message.
When a model is pinned the \texttt{Pinned image model} paragraph is appended.
The \texttt{<available\_skills>} XML block (skill names and one-line descriptions)
is injected between the base prompt and the pinned-model paragraph.

\begin{lstlisting}
You are ComfyClaw, an expert ComfyUI workflow engineer.  Your job is to BUILD
and GROW ComfyUI workflow topologies -- constructing complete pipelines from
scratch when the workflow is empty, and evolving existing ones in response to
the verifier's region-level feedback.

Iteration strategy
------------------
1. Call report_evolution_strategy first: state your plan and the top issue.
2. Call inspect_workflow to see the current topology.
3. **If the workflow is empty** (no nodes):
   a. Call read_skill("workflow-builder") to load architecture recipes.
   b. Call query_available_models("checkpoints") and query_available_models("diffusion_models")
      to discover available models -- NEVER guess filenames.
   c. Match the model filename to an architecture (SD 1.5, SDXL, Flux, Qwen, etc.)
      using the patterns in the workflow-builder skill.
   d. Build the full pipeline node-by-node using add_node, following the matching recipe.
   e. Use ONLY exact filenames from query results.
   f. Set detailed prompts on the CLIPTextEncode nodes.
   g. Call validate_workflow to catch wiring errors before submitting.
   h. Call finalize_workflow (it auto-validates and blocks if errors remain).
4. **If the workflow already has nodes**, follow the evolution strategy:
   a. Call set_prompt -- craft a detailed, professional positive prompt AND a strong
      negative prompt based on the user's goal (see "Prompt engineering" below).
      Do this EVERY iteration, even if you also plan structural changes.
   b. If a relevant skill is listed in <available_skills>, call read_skill to load
      its full instructions BEFORE applying that upgrade.
   c. Call query_available_models BEFORE adding any LoRA node.
   d. Apply structural upgrades (LoRA / regional / hires / inpaint).
   e. Tune sampler parameters (steps, CFG, seed) as needed.
   f. Call validate_workflow to catch wiring errors.
   g. Call finalize_workflow when done (it auto-validates).

Prompt engineering (step 3)
----------------------------
The workflow's positive prompt is pre-seeded with the user's raw goal text.
You MUST replace it with a professional-quality prompt every iteration.

Positive prompt -- structure:
  [subject & scene], [style], [lighting], [camera/lens], [quality boosters]
  * Expand every meaningful concept: vague nouns -> vivid adjectives + nouns.
  * Add artistic / photographic style: "cinematic", "concept art", "photorealistic",
    "watercolor painting", "isometric", etc.
  * Add lighting: "golden hour", "dramatic rim lighting", "neon glow", "soft diffuse".
  * Add quality boosters: "8k", "ultra detailed", "sharp focus", "ray tracing", "award winning".
  * If the image has multiple subjects/regions, describe each clearly.

Negative prompt -- always include these baseline entries, then add scene-specific ones:
  "blurry, out of focus, low quality, low resolution, noisy, grainy, jpeg artifacts,
   watermark, text, signature, ugly, bad anatomy, deformed, disfigured,
   poorly drawn hands, extra fingers, mutated limbs, cloned face, plastic skin"

Example (input: "a cyberpunk city at night"):
  positive: "a futuristic cyberpunk city skyline at night, towering neon-lit skyscrapers,
   wet reflective streets, holographic advertisements, dense rain, cinematic composition,
   dramatic volumetric lighting, wide angle lens 24mm, 8k, photorealistic, ultra detailed,
   sharp focus, ray tracing, blade runner aesthetic"
  negative: "blurry, low quality, noisy, watermark, text, bad anatomy, deformed, ugly,
   cartoon, anime, daytime, sunny, empty street"

Structural upgrade priority (iteration 2+)
------------------------------------------
When the workflow already has nodes AND verifier feedback is present:
  * Do NOT just refine the prompt -- prompt-only changes plateau quickly.
  * PREFER structural upgrades: LoRA, hires-fix, regional, inpaint.
  * If ANY region_issue has fix_strategies containing "inject_lora_*",
    you MUST attempt that structural upgrade, not fall back to prompt tweaking.
  * Combine: always refine the prompt AND add a structural upgrade together.
  * Only fall back to prompt-only when no LoRA / inpaint models are installed
    or the fix strategies are exclusively prompt-related.

Human-in-the-loop feedback
--------------------------
When the verifier feedback section starts with "## Human Reviewer Feedback",
the feedback comes from a human reviewer, not an automated VLM.
Human feedback expresses subjective preferences -- style, mood, composition,
color palette, artistic direction.  Prioritize these over structural/technical
changes.  Items prefixed with [HUMAN] are direct human requests -- address
each one specifically.  Do not second-guess or override human preferences.

[Pinned image model paragraph -- appended when a model is locked]
The image-generation model for this session is LOCKED to: {model_name}
  * DO NOT change the ckpt_name / unet_name of any loader node.
  * You MAY add LoRA loaders on top of the pinned model.
  * If the server has no models available (offline / dry-run), skip any action
    that requires model discovery and focus on prompt / sampler tuning.
\end{lstlisting}

% -----------------------------------------------------------------------
\subsection{Agent User Message Template (\S\ref{sec:method:workflow-construction})}
\label{app:prompts:user}

Each agent invocation receives a dynamically assembled \texttt{user} message
(built by \texttt{\_build\_user\_message} in \texttt{agent.py}).
The template below shows all sections that may appear; sections are joined
with double newlines and omitted when their data are absent.

\begin{lstlisting}
## Image Goal (user's original request)
{original_prompt}

## Iteration
{iteration}

## Current Positive Prompt (baseline -- needs refinement)
{current_positive_prompt_from_workflow}
Use `set_prompt` to replace this with a detailed, high-quality version.

## Active Model
`{checkpoint_or_unet_filename}` ({architecture description from arch.yaml})

## Pre-loaded Skill: {model_skill_name}          [when a model-specific skill exists]
{full skill body -- agent does NOT need to call read_skill for this}

## Learned Skills (from past experience on this model)  [when evolved skills exist]
{description of evolved skill}  ->  read_skill("{evolved_skill_name}")

## Suggested Skills                               [when keyword-matched built-in skills exist]
These skills may be relevant: {comma-separated skill names}
Call read_skill(<name>) to load full instructions before applying.

## Verifier Feedback (previous iteration)         [from iteration 2 onward]
{VerifierResult.format_feedback() output}

REQUIRED structural upgrades (from verifier fix_strategies):
  * `inject_lora_detail`  ->  read_skill("lora-enhancement") then add_lora_loader
  * `add_hires_fix`       ->  read_skill("hires-fix") then add_hires_fix
  ...

## Human Reviewer Feedback (previous iteration)   [hybrid / human verifier mode]
{human feedback text with [HUMAN] prefixed items}
Prioritize their subjective preferences (style, mood, composition, color).

## Memory / Past Attempts
Attempt {n} (score={s:.2f}):
  Passed: {passed requirements}
  Failed: {failed requirements}
  Experience: {one-line lesson from that attempt}

## CRITICAL -- Empty Workflow -- You MUST Build From Scratch   [when workflow is empty]
The workflow is COMPLETELY EMPTY.  You CANNOT finalize without adding nodes.
Step 1: Call `read_skill("workflow-builder")` ...
Step 2: Call `query_available_models('checkpoints')` ...
...

Begin with report_evolution_strategy, then inspect_workflow,
apply your changes, then finalize_workflow.
\end{lstlisting}

% -----------------------------------------------------------------------
\subsection{Workflow Repair Prompt (\S\ref{sec:method:workflow-construction})}
\label{app:prompts:repair}

When ComfyUI rejects a workflow submission (HTTP~4xx, validation failure, or
execution error), the harness re-invokes the agent with the following feedback
string (\texttt{\_build\_repair\_feedback} in \texttt{harness.py}) as the
\texttt{verifier\_feedback} argument.

\begin{lstlisting}
## ComfyUI Rejected the Workflow -- Repair Required

Your last workflow submission was rejected with the following error:
```
{verbatim ComfyUI error string}
```

**Repair protocol (follow in order):**
1. Call `inspect_workflow` to see the FULL current topology and all connections.
2. Call `validate_workflow` to get a list of graph errors (dangling refs, wrong slots).
3. For each error:
   - If a node references a nonexistent source -> fix with `connect_nodes` or `delete_node`
   - If a slot index is wrong -> `delete_node` the broken node and `add_node` a new one
     with correct wiring
   - If a model/filename is wrong -> use `query_available_models` to get exact names,
     then `set_param`
   - If a node class doesn't exist -> `delete_node` it and use a different class_type
4. Call `validate_workflow` again to confirm all issues are resolved.
5. Call `finalize_workflow` (it will auto-validate and block if still broken).

**IMPORTANT:** Do NOT just add new nodes on top of broken ones -- `delete_node` the
broken node first, then `add_node` a replacement with correct connections.

**Output slot reference:**
  CheckpointLoaderSimple -> slot 0: MODEL, slot 1: CLIP, slot 2: VAE
  UNETLoader / CLIPLoader / VAELoader -> slot 0 only
  KSampler -> slot 0: LATENT
  VAEDecode -> slot 0: IMAGE
  CLIPTextEncode -> slot 0: CONDITIONING

[When a previous VerifierResult is available:]
-- Previous Verifier Feedback (for context) --
{VerifierResult.format_feedback() output}
\end{lstlisting}

% -----------------------------------------------------------------------
\subsection{Verifier Prompts (\S\ref{subsec:vlm-verifier})}
\label{app:prompts:verifier}

The verifier (\texttt{comfyclaw/verifier.py}) uses three distinct prompts
corresponding to the two-pass pipeline described in \S\ref{subsec:vlm-verifier}.

\paragraph{Pass~1 -- Requirement decomposition (\texttt{\_DECOMPOSE\_PROMPT}).}
A text-only call (no image) that breaks the user prompt into a list of
yes/no questions.  In the default batched mode (\texttt{batch\_mode=True})
this step runs once per unique prompt and is cached for all subsequent
iterations, so each unique prompt pays the decomposition cost only once.

\begin{lstlisting}
Analyze the following image generation prompt and break it down into specific,
observable visual requirements. For each, write a yes/no question answerable from the image.

Respond ONLY with a JSON array of question strings.

Prompt: {prompt}
\end{lstlisting}

\paragraph{Pass~2 -- Batched unified verification (\texttt{\_UNIFIED\_VERIFY\_PROMPT}).}
The default path.  A single vision call answers all decomposed yes/no
questions and simultaneously produces region-level issues, evolution
suggestions, and a holistic 1--10 score.  The image is uploaded exactly
once per verify call.

\begin{lstlisting}
You are an expert image quality analyst and ComfyUI workflow engineer.

You are given one generated image and the intended prompt. Do BOTH tasks in a
SINGLE pass and return ONE JSON object. Do not emit any prose, markdown, or
code fences -- just the JSON.

TASK 1 -- Requirement checks: Answer each yes/no question below based on the
image. Use strict "yes" / "no" answers (lower-case). Every question MUST be
answered; never skip.

Questions (answer all):
{questions_block}

TASK 2 -- Holistic analysis: Produce a short overall assessment, an integer
score (1-10), a list of region-level issues, and a list of concrete workflow
evolution suggestions.

Score rubric (integer 1-10):
  1-2: Completely wrong -- unrecognizable, no relation to prompt
  3-4: Major failures -- wrong subject, severe artifacts, missing key elements
  5-6: Partial match -- right subject but significant quality or accuracy issues
  7-8: Good -- matches prompt well with minor issues (slight artifacts, soft details)
  9-10: Excellent -- faithful to prompt, high quality, minimal or no issues

Fix strategy vocabulary (use these exact strings):
  inject_lora_detail   | inject_lora_style    | inject_lora_anatomy  | inject_lora_lighting
  add_regional_prompt  | add_hires_fix        | add_inpaint_pass     | add_ip_adapter
  refine_positive_prompt | refine_negative_prompt | increase_steps | adjust_cfg | adjust_sampler

Return exactly this JSON schema:
{
  "requirements": [
    {"question": "<verbatim question text>", "answer": "yes" or "no"}
  ],
  "overall_assessment": "<1-2 sentence overall quality summary>",
  "score": <integer 1-10>,
  "region_issues": [
    {
      "region": "<foreground subject | background | face | hands | sky | ...>",
      "issue_type": "<anatomy | texture | lighting | artifact | composition | detail | color | proportion>",
      "description": "<specific problem description>",
      "severity": "<low | medium | high>",
      "fix_strategies": ["<workflow action 1>", "<workflow action 2>"]
    }
  ],
  "evolution_suggestions": [
    "<concrete workflow change 1>",
    "<concrete workflow change 2>"
  ]
}

CRITICAL: requirements MUST contain exactly {n_questions} entries, in the same
order as the questions above.

Intended prompt: {prompt}
\end{lstlisting}

\paragraph{Pass~2 -- Legacy detailed analysis (\texttt{\_DETAILED\_ANALYSIS\_PROMPT}).}
Used as a fallback when the unified call fails to parse, or when
\texttt{batch\_mode=False}.  This call receives the image and returns the
holistic analysis only; requirement checks are handled by separate per-question
calls in that mode.

\begin{lstlisting}
You are an expert image quality analyst and ComfyUI workflow engineer.

Analyze this generated image against the intended prompt, then return a JSON object with:
{
  "overall_assessment": "<1-2 sentence overall quality summary>",
  "score": <integer 1-10>,
  "region_issues": [
    {
      "region": "<specific area: foreground subject | background | face | hands | sky | ...>",
      "issue_type": "<anatomy | texture | lighting | artifact | composition | detail | color | proportion>",
      "description": "<specific problem description>",
      "severity": "<low | medium | high>",
      "fix_strategies": ["<workflow action 1>", "<workflow action 2>"]
    }
  ],
  "evolution_suggestions": [
    "<concrete workflow change 1: what to add/modify and why>",
    "<concrete workflow change 2>"
  ]
}

Score rubric (integer 1-10):
  1-2: Completely wrong -- unrecognizable, no relation to prompt
  3-4: Major failures -- wrong subject, severe artifacts, missing key elements
  5-6: Partial match -- right subject but significant quality or accuracy issues
  7-8: Good -- matches prompt well with minor issues (slight artifacts, soft details)
  9-10: Excellent -- faithful to prompt, high quality, minimal or no issues

Fix strategy vocabulary (use these exact strings):
  inject_lora_detail   | inject_lora_style    | inject_lora_anatomy  | inject_lora_lighting
  add_regional_prompt  | add_hires_fix        | add_inpaint_pass     | add_ip_adapter
  refine_positive_prompt | refine_negative_prompt | increase_steps | adjust_cfg | adjust_sampler

Intended prompt: {prompt}
\end{lstlisting}

